Explainable Software Defect Prediction: Are We There Yet?

Explaining the prediction results of software defect prediction models is a challenging while practical task, which can provide useful information for developers to understand and fix the predicted bugs. To address this issue, recently, Jiarpakdee et al. proposed to use {two state-of-the-art} model-agnostic techniques (i.e., LIME and BreakDown) to explain the prediction results of bug prediction models. Their experiments show these tools can generate promising results and the generated explanations can assist developers understand the prediction results. However, the fact that LIME and BreakDown were only examined on a single software defect prediction model setting calls into question about their consistency and reliability across software defect prediction models with various settings. In this paper, we set out to investigate the consistency and reliability of model-agnostic technique based explanation generation approaches (i.e., LIME and BreakDown) on software defect prediction models with different settings , e.g., different data sampling techniques, different machine learning classifiers, and different prediction scenarios. Specifically, we use both LIME and BreakDown to generate explanations for the same instance under software defect prediction models with different settings and then check the consistency of the generated explanations for the instance. We reused the same defect data from Jiarpakdee et al. in our experiments. The results show that both LIME and BreakDown generate inconsistent explanations under different software defect prediction settings for the same test instances, which makes them unreliable for explanation generation. Overall, with this study, we call for more research in explainable software defect prediction towards achieving consistent and reliable explanation generation.

==> TSE - Explainable Software Defect Prediction_ Are We There Yet_/figure/diff_n/diff_n.tex <==
\begin{figure*}[t!]
\centering 
\begin{subfigure}{ 0.25\linewidth}
\centering
\includegraphics[width=\textwidth]{figure/diff_n/diff_n_lime_hr.png}
%\vspace{-0.2in}
\caption{\small {\hitrate} of \emph{LIME}}
%\vspace{-0.1in}
\end{subfigure}\hfill
\begin{subfigure}{ 0.25\linewidth}
\centering
\includegraphics[width=\textwidth]{figure/diff_n/diff_n_lime_rd.png}
%\vspace{-0.2in}
\caption{\small {\rd} of \emph{LIME}}
%\vspace{-0.1in}
\end{subfigure}\hfill
\begin{subfigure}{ 0.25\linewidth}
\centering
\includegraphics[width=\textwidth]{figure/diff_n/diff_n_bd_hr.png}
%\vspace{-0.2in}
\caption{\small{ {\hitrate}} of \emph{BreakDown}}
%\vspace{-0.1in}
\end{subfigure}\hfill
\begin{subfigure}{ 0.25\linewidth}
\centering
\includegraphics[width=\textwidth]{figure/diff_n/diff_n_bd_rd.png}
%\vspace{-0.2in}
\caption{\small{ {\rd}} of \emph{BreakDown}}
%\vspace{-0.1in}
\end{subfigure}\hfill

\vspace{-0.1in}
\caption{
The distributions of {\hitrate} and {\rd} of \emph{LIME} and \emph{BreakDown} with different top-N features.}
\label{fig:diff_n}
%\vspace{-0.1in}
\end{figure*}
%\vspace{-0.1in}


==> TSE - Explainable Software Defect Prediction_ Are We There Yet_/figure/motivation.tex <==
\begin{figure*}[t!]
     \centering
     \begin{subfigure}[b]{0.49\textwidth}
         \centering
         \includegraphics[width=1\textwidth]{figure/motiv_ex_1.png}
         \caption{Explanation with LR-based defect prediction model} 
         %{\song{why CoutLine is not the first selected feature as it has the largest value?}}
         %\jiho{because value indicates to the actual value of the feature, not the points that it accounts to the rankings.}}
         \label{fig:motiv_ex_1}
     \end{subfigure}
     \begin{subfigure}[b]{0.49\textwidth}
         \centering
         \includegraphics[width=1\textwidth]{figure/motiv_ex_2.png}
         \caption{Explanation with DT-based defect prediction model}
         \label{fig:motiv_ex_2}
     \end{subfigure}
     \hfill
        \caption{%{%\jiho{Fig. 1. Updated}}
        Explanations generated by LIME for the predicted buggy file \textit{``ActiveMQConnection.java''} from project activemq-5.0.0 with different defect prediction models.}
        \label{fig:motiv_ex}
\end{figure*}

==> TSE - Explainable Software Defect Prediction_ Are We There Yet_/figure/rq1/rq1_combine.tex <==
\begin{figure*}[th!]
\centering
\begin{subfigure}{0.24\linewidth}
\centering
\input{figure/rq1/vt_lime_hr}
\vspace{-0.2in}
\caption{\emph{LIME} {\hitrate}}
%\vspace{-0.1in}
\end{subfigure}\hfill
\begin{subfigure}{0.24\linewidth}
\centering
\input{figure/rq1/vt_bd_hr}
\vspace{-0.2in}
\caption{\emph{BreakDown} {\hitrate}}
%\vspace{-0.1in}
\end{subfigure}\hfill
\begin{subfigure}{0.24\linewidth}
\centering
\input{figure/rq1/vt_lime_rd}
\vspace{-0.2in}
\caption{\emph{LIME} {\rd}}
%\vspace{-0.1in}
\end{subfigure}\hfill
\begin{subfigure}{0.24\linewidth}
\centering
\input{figure/rq1/vt_bd_rd}
\vspace{-0.2in}
\caption{\emph{BreakDown} {\rd}}
%\vspace{-0.1in}
\end{subfigure}\hfill

\centering
\begin{subfigure}{0.24\linewidth}
\centering
\input{figure/rq1/svc_lime_hr}
\vspace{-0.2in}
\caption{\emph{LIME} {\hitrate}}
%\vspace{-0.1in}
\end{subfigure}\hfill
\begin{subfigure}{0.24\linewidth}
\centering
\input{figure/rq1/svc_bd_hr}
\vspace{-0.2in}
\caption{\emph{BreakDown} {\hitrate}}
%\vspace{-0.1in}
\end{subfigure}\hfill
\begin{subfigure}{0.24\linewidth}
\centering
\input{figure/rq1/svc_lime_rd}
\vspace{-0.2in}
\caption{\emph{LIME} {\rd}}
%\vspace{-0.1in}
\end{subfigure}\hfill
\begin{subfigure}{0.24\linewidth}
\centering
\input{figure/rq1/svc_bd_rd}
\vspace{-0.2in}
\caption{\emph{BreakDown} {\rd}}
%\vspace{-0.1in}
\end{subfigure}\hfill

\centering
\begin{subfigure}{0.24\linewidth}
\centering
\input{figure/rq1/fpr_lime_hr}
\vspace{-0.2in}
\caption{\emph{LIME} {\hitrate}}
%\vspace{-0.1in}
\end{subfigure}\hfill
\begin{subfigure}{0.24\linewidth}
\centering
\input{figure/rq1/fpr_bd_hr}
\vspace{-0.2in}
\caption{\emph{BreakDown} {\hitrate}}
%\vspace{-0.1in}
\end{subfigure}\hfill
\begin{subfigure}{0.24\linewidth}
\centering
\input{figure/rq1/fpr_lime_rd}
\vspace{-0.2in}
\caption{\emph{LIME} {\rd}}
%\vspace{-0.1in}
\end{subfigure}\hfill
\begin{subfigure}{0.24\linewidth}
\centering
\input{figure/rq1/fpr_bd_rd}
\vspace{-0.2in}
\caption{\emph{BreakDown} {\rd}}
%\vspace{-0.1in}
\end{subfigure}\hfill

\vspace{-0.1in}
\caption{ \small
This is the {\hitrate} and {\rd} comparison of different feature selection method applied.
(a) $\sim$ (d) is the result of Variance Threshold Feature Selection Method.
(e) $\sim$ (h) is the result of SelectFromModel (L1 norm) Feature Selection Method.
(i) $\sim$ (l) is the result of Univariate Feature Selection Method (FPR).
}
\label{fig:rq1_comb}
\vspace{-0.1in}
\end{figure*}
%\vspace{-0.1in}


==> TSE - Explainable Software Defect Prediction_ Are We There Yet_/figure/rq2/rq2_combine.tex <==
\begin{figure*}[th!]

\centering 
\begin{subfigure}{0.20\linewidth}
\centering
\includegraphics[width=\textwidth]{figure/rq2/rq2_cc_lime_hr.png}
\vspace{-0.05in}
\caption{Cluster Centroids}
%\vspace{-0.05in}
\end{subfigure}\hfill
\begin{subfigure}{0.20\linewidth}
\centering
\includegraphics[width=\textwidth]{figure/rq2/rq2_renn_lime_hr.png}
\vspace{-0.05in}
\caption{RENN}
%\vspace{-0.05in}
\end{subfigure}\hfill
\begin{subfigure}{0.20\linewidth}
\centering
\includegraphics[width=\textwidth]{figure/rq2/rq2_rus_lime_hr.png}
\vspace{-0.05in}
\caption{RUS}
%\vspace{-0.05in}
\end{subfigure}\hfill
\centering
\begin{subfigure}{0.20\linewidth}
\centering
\includegraphics[width=\textwidth]{figure/rq2/rq2_ros_lime_hr.png}
\vspace{-0.05in}
\caption{ROS}
%\vspace{-0.05in}
\end{subfigure}\hfill
\centering
\begin{subfigure}{0.20\linewidth}
\centering
\includegraphics[width=\textwidth]{figure/rq2/rq2_smote_lime_hr.png}
\vspace{-0.05in}
\caption{SMOTE}
%\vspace{-0.05in}
\end{subfigure}\hfill

\centering 
\begin{subfigure}{0.20\linewidth}
\centering
\includegraphics[width=\textwidth]{figure/rq2/rq2_cc_lime_rd.png}
\vspace{-0.05in}
\caption{Cluster Centroids}
%\vspace{-0.05in}
\end{subfigure}\hfill
\begin{subfigure}{0.20\linewidth}
\centering
\includegraphics[width=\textwidth]{figure/rq2/rq2_renn_lime_rd.png}
\vspace{-0.05in}
\caption{RENN}
%\vspace{-0.05in}
\end{subfigure}\hfill
\begin{subfigure}{0.20\linewidth}
\centering
\includegraphics[width=\textwidth]{figure/rq2/rq2_rus_lime_rd.png}
\vspace{-0.05in}
\caption{RUS}
%\vspace{-0.05in}
\end{subfigure}\hfill
\centering
\begin{subfigure}{0.20\linewidth}
\centering
\includegraphics[width=\textwidth]{figure/rq2/rq2_ros_lime_rd.png}
\vspace{-0.05in}
\caption{ROS}
%\vspace{-0.05in}
\end{subfigure}\hfill
\centering
\begin{subfigure}{0.20\linewidth}
\centering
\includegraphics[width=\textwidth]{figure/rq2/rq2_smote_lime_rd.png}
\vspace{-0.05in}
\caption{SMOTE}
%\vspace{-0.05in}
\end{subfigure}\hfill

\centering 
\begin{subfigure}{0.20\linewidth}
\centering
\includegraphics[width=\textwidth]{figure/rq2/rq2_cc_bd_hr.png}
\vspace{-0.05in}
\caption{Cluster Centroids}
%\vspace{-0.05in}
\end{subfigure}\hfill
\begin{subfigure}{0.20\linewidth}
\centering
\includegraphics[width=\textwidth]{figure/rq2/rq2_renn_bd_hr.png}
\vspace{-0.05in}
\caption{RENN}
%\vspace{-0.05in}
\end{subfigure}\hfill
\begin{subfigure}{0.20\linewidth}
\centering
\includegraphics[width=\textwidth]{figure/rq2/rq2_rus_bd_hr.png}
\vspace{-0.05in}
\caption{RUS}
%\vspace{-0.05in}
\end{subfigure}\hfill
\centering
\begin{subfigure}{0.20\linewidth}
\centering
\includegraphics[width=\textwidth]{figure/rq2/rq2_ros_bd_hr.png}
\vspace{-0.05in}
\caption{ROS}
%\vspace{-0.05in}
\end{subfigure}\hfill
\centering
\begin{subfigure}{0.20\linewidth}
\centering
\includegraphics[width=\textwidth]{figure/rq2/rq2_smote_bd_hr.png}
\vspace{-0.05in}
\caption{SMOTE}
%\vspace{-0.05in}
\end{subfigure}\hfill

\centering 
\begin{subfigure}{0.20\linewidth}
\centering
\includegraphics[width=\textwidth]{figure/rq2/rq2_cc_bd_rd.png}
\vspace{-0.05in}
\caption{Cluster Centroids}
%\vspace{-0.05in}
\end{subfigure}\hfill
\begin{subfigure}{0.20\linewidth}
\centering
\includegraphics[width=\textwidth]{figure/rq2/rq2_renn_bd_rd.png}
\vspace{-0.05in}
\caption{RENN}
%\vspace{-0.05in}
\end{subfigure}\hfill
\begin{subfigure}{0.20\linewidth}
\centering
\includegraphics[width=\textwidth]{figure/rq2/rq2_rus_bd_rd.png}
\vspace{-0.05in}
\caption{RUS}
%\vspace{-0.05in}
\end{subfigure}\hfill
\centering
\begin{subfigure}{0.20\linewidth}
\centering
\includegraphics[width=\textwidth]{figure/rq2/rq2_ros_bd_rd.png}
\vspace{-0.05in}
\caption{ROS}
%\vspace{-0.05in}
\end{subfigure}\hfill
\centering
\begin{subfigure}{0.20\linewidth}
\centering
\includegraphics[width=\textwidth]{figure/rq2/rq2_smote_bd_rd.png}
\vspace{-0.05in}
\caption{SMOTE}
%\vspace{-0.05in}
\end{subfigure}\hfill
%\vspace{-0.05in}
\caption{{The distributions of {\hitrate} and {\rd} on each project before and after applying data sampling techniques. 
(a) $\sim$ (e) is the result of {\hitrate} of \emph{LIME}.
(f) $\sim$ (j) is the result of {\rd} of \emph{LIME}.
(k) $\sim$ (o) is the result of {\hitrate} of \emph{BreakDown}.
(p) $\sim$ (t) is the result of {\rd} of \emph{BreakDown}.}}
\label{fig:rq2_comb}
%\vspace{-0.05in}
\end{figure*}
%\vspace{-0.05in}


==> TSE - Explainable Software Defect Prediction_ Are We There Yet_/figure/rq3.tex <==
\begin{figure}
\captionsetup[subfigure]{justification=centering}
    % hit rate part of figure
    \begin{subfigure}[]{\linewidth}
        \begin{tikzpicture}
        \begin{axis}[
        ymax=2,
        ymin=0,
        y=1.5cm,
        xtick={0.0,0.2,0.4,0.6,0.8,1.0},
        xticklabels={0.0,0.2,0.4,0.6,0.8,1.0},
        ytick={1},
        yticklabels={\qquad \, LIME},
        axis y line=left,
        axis x line=bottom,
        xmin=0.0,
        xmax=1.0,
        %ytick={1,2,3},
        %yticklabels={Group A, Group B, Group C},
        ]
        \addplot+[black,thick,
        boxplot prepared={
            draw position=1,
            lower whisker=0.320,
            lower quartile=0.488,
            median=0.541,
            upper quartile=0.629,
            upper whisker=0.791,
        },/pgf/number format/precision=0
        ]
        coordinates {}
        [above]
        node at
        (boxplot box cs: \boxplotvalue{lower whisker},1){}
        node at
        (boxplot box cs: \boxplotvalue{lower quartile},1){}
        node at
        (boxplot box cs: \boxplotvalue{median},1){}
        node at
        (boxplot box cs: \boxplotvalue{upper quartile},1){}
        node at
        (boxplot box cs: \boxplotvalue{upper whisker},1){}
        ;
        
        \end{axis}
        \end{tikzpicture}
        \caption{{\hitrate} of \emph{LIME}}
        \label{fig:rq3_hitrate}
        
    \end{subfigure}

    % rank_diff part of figure
    \begin{subfigure}[]{\linewidth}
        \begin{tikzpicture}
        \begin{axis}[
        ymax=3.5,
        ymin=0,
        y=1.5cm,
        xtick={3,6,...,23},
        xticklabels={3,6,...,23},
        ytick={1,2.5},
        yticklabels={BreakDown, LIME},
        axis y line=left,
        axis x line=bottom,
        xmin=3,
        xmax=23,
        %ytick={1,2,3},
        %yticklabels={Group A, Group B, Group C},
        ]
        \addplot+[black,thick,
        boxplot prepared={
            draw position=2.5,
            lower whisker=3.357,
            lower quartile=4.765,
            median=5.834,
            upper quartile=6.322,
            upper whisker=7.291,
        },/pgf/number format/precision=0
        ]
        coordinates {}
        [above]
        node at
        (boxplot box cs: \boxplotvalue{lower whisker},1){}
        node at
        (boxplot box cs: \boxplotvalue{lower quartile},1){}
        node at
        (boxplot box cs: \boxplotvalue{median},1){}
        node at
        (boxplot box cs: \boxplotvalue{upper quartile},1){}
        node at
        (boxplot box cs: \boxplotvalue{upper whisker},1){}
        ;
         \addplot+[black,thick,
        boxplot prepared={
            draw position=1,
            lower whisker=3.940,
            lower quartile=10.106,
            median=12.444,
            upper quartile=14.698,
            upper whisker=18.923,
        },/pgf/number format/precision=0
        ]
        coordinates {(1,22.913) (1,24.919)}
        [above]
        node at
        (boxplot box cs: \boxplotvalue{lower whisker},1){}
        node at
        (boxplot box cs: \boxplotvalue{lower quartile},1){}
        node at
        (boxplot box cs: \boxplotvalue{median},1){}
        node at
        (boxplot box cs: \boxplotvalue{upper quartile},1){}
        node at
        (boxplot box cs: \boxplotvalue{upper whisker},1){}
        ;
        \end{axis}
        \end{tikzpicture}
        \caption{{\rankdiff} of \emph{LIME} and \emph{BreakDown}}
        \label{fig:rq3_rankdiff}
    \end{subfigure}
    \caption{Result of RQ3, comparing explanations in cross-version defect prediction scenario}
    \label{fig:rq3}
\end{figure}


==> TSE - Explainable Software Defect Prediction_ Are We There Yet_/figure/rq3/rq3_combine.tex <==
\begin{figure*}[th!]

\centering 
\begin{subfigure}{0.20\linewidth}
\centering
\includegraphics[width=\textwidth]{figure/rq3/rq3_dt_lime_hr.png}
\vspace{-0.2in}
\caption{Decision Tree}
%\vspace{-0.1in}
\end{subfigure}\hfill
\begin{subfigure}{0.20\linewidth}
\centering
\includegraphics[width=\textwidth]{figure/rq3/rq3_ens_lime_hr.png}
\vspace{-0.2in}
\caption{Ensemble}
%\vspace{-0.1in}
\end{subfigure}\hfill
\begin{subfigure}{0.20\linewidth}
\centering
\includegraphics[width=\textwidth]{figure/rq3/rq3_gnb_lime_hr.png}
\vspace{-0.2in}
\caption{NaiveBayes}
%\vspace{-0.1in}
\end{subfigure}\hfill
\centering
\begin{subfigure}{0.20\linewidth}
\centering
\includegraphics[width=\textwidth]{figure/rq3/rq3_rf_lime_hr.png}
\vspace{-0.2in}
\caption{RandomForest}
%\vspace{-0.1in}
\end{subfigure}\hfill
\centering
\begin{subfigure}{0.20\linewidth}
\centering
\includegraphics[width=\textwidth]{figure/rq3/rq3_dt_lime_hr.png}
\vspace{-0.2in}
\caption{SVM}
%\vspace{-0.1in}
\end{subfigure}\hfill

\centering 
\begin{subfigure}{0.20\linewidth}
\centering
\includegraphics[width=\textwidth]{figure/rq3/rq3_dt_lime_rd.png}
\vspace{-0.2in}
\caption{Decision Tree}
%\vspace{-0.1in}
\end{subfigure}\hfill
\begin{subfigure}{0.20\linewidth}
\centering
\includegraphics[width=\textwidth]{figure/rq3/rq3_ens_lime_rd.png}
\vspace{-0.2in}
\caption{Ensemble}
%\vspace{-0.1in}
\end{subfigure}\hfill
\begin{subfigure}{0.20\linewidth}
\centering
\includegraphics[width=\textwidth]{figure/rq3/rq3_gnb_lime_rd.png}
\vspace{-0.2in}
\caption{NaiveBayes}
%\vspace{-0.1in}
\end{subfigure}\hfill
\centering
\begin{subfigure}{0.20\linewidth}
\centering
\includegraphics[width=\textwidth]{figure/rq3/rq3_rf_lime_rd.png}
\vspace{-0.2in}
\caption{RandomForest}
%\vspace{-0.1in}
\end{subfigure}\hfill
\centering
\begin{subfigure}{0.20\linewidth}
\centering
\includegraphics[width=\textwidth]{figure/rq3/rq3_svc_lime_rd.png}
\vspace{-0.2in}
\caption{SVM}
%\vspace{-0.1in}
\end{subfigure}\hfill

\centering 
\begin{subfigure}{0.20\linewidth}
\centering
\includegraphics[width=\textwidth]{figure/rq3/rq3_dt_bd_rd.png}
\vspace{-0.2in}
\caption{Decision Tree}
%\vspace{-0.1in}
\end{subfigure}\hfill
\begin{subfigure}{0.20\linewidth}
\centering
\includegraphics[width=\textwidth]{figure/rq3/rq3_ens_bd_rd.png}
\vspace{-0.2in}
\caption{Ensemble}
%\vspace{-0.1in}
\end{subfigure}\hfill
\begin{subfigure}{0.20\linewidth}
\centering
\includegraphics[width=\textwidth]{figure/rq3/rq3_gnb_bd_rd.png}
\vspace{-0.2in}
\caption{NaiveBayes}
%\vspace{-0.1in}
\end{subfigure}\hfill
\centering
\begin{subfigure}{0.20\linewidth}
\centering
\includegraphics[width=\textwidth]{figure/rq3/rq3_rf_bd_rd.png}
\vspace{-0.2in}
\caption{RandomForest}
%\vspace{-0.1in}
\end{subfigure}\hfill
\centering
\begin{subfigure}{0.20\linewidth}
\centering
\includegraphics[width=\textwidth]{figure/rq3/rq3_svc_bd_rd.png}
\vspace{-0.2in}
\caption{SVM}
%\vspace{-0.1in}
\end{subfigure}\hfill


\vspace{-0.1in}
\caption{ \small
The distributions of {\hitrate} and {\rd} on each project before and after applying data sampling techniques. 
(a) $\sim$ (e) is the result of {\hitrate} of \emph{LIME}.
(f) $\sim$ (j) is the result of {\rd} of \emph{LIME}.
(k) $\sim$ (o) is the result of {\rd} of \emph{BreakDown}.
}
\label{fig:rq3_comb}
\vspace{-0.1in}
\end{figure*}
%\vspace{-0.1in}


==> TSE - Explainable Software Defect Prediction_ Are We There Yet_/figure/rq4.tex <==
\begin{figure}
\captionsetup[subfigure]{justification=centering}
    % hit rate part of figure
    \begin{subfigure}[]{\linewidth}
        \begin{tikzpicture}
        \begin{axis}[
        ymax=2,
        ymin=0,
        y=1.5cm,
        xtick={0.0,0.2,0.4,0.6,0.8,1.0},
        xticklabels={0.0,0.2,0.4,0.6,0.8,1.0},
        ytick={1},
        yticklabels={\qquad \, LIME},
        axis y line=left,
        axis x line=bottom,
        xmin=0.0,
        xmax=1.0,
        %ytick={1,2,3},
        %yticklabels={Group A, Group B, Group C},
        ]
        \addplot+[black,thick,
        boxplot prepared={
            draw position=1,
            lower whisker=0.130,
            lower quartile=0.331,
            median=0.549,
            upper quartile=0.624,
            upper whisker=0.810,
        },/pgf/number format/precision=0
        ]
        coordinates {}
        [above]
        node at
        (boxplot box cs: \boxplotvalue{lower whisker},1){}
        node at
        (boxplot box cs: \boxplotvalue{lower quartile},1){}
        node at
        (boxplot box cs: \boxplotvalue{median},1){}
        node at
        (boxplot box cs: \boxplotvalue{upper quartile},1){}
        node at
        (boxplot box cs: \boxplotvalue{upper whisker},1){}
        ;
        
        \end{axis}
        \end{tikzpicture}
        \caption{{\hitrate} of \emph{LIME}}
        \label{fig:rq4_hitrate}
        
    \end{subfigure}

    % rank_diff part of figure
    \begin{subfigure}[]{\linewidth}
        \begin{tikzpicture}
        \begin{axis}[
        ymax=3.5,
        ymin=0,
        y=1.5cm,
        xtick={3,6,...,23},
        xticklabels={3,6,...,23},
        ytick={1,2.5},
        yticklabels={BreakDown, LIME},
        axis y line=left,
        axis x line=bottom,
        xmin=3,
        xmax=23,
        %ytick={1,2,3},
        %yticklabels={Group A, Group B, Group C},
        ]
        \addplot+[black,thick,
        boxplot prepared={
            draw position=2.5,
            lower whisker=3.567,
            lower quartile=5.035,
            median=5.819,
            upper quartile=7.256,
            upper whisker=9.134,
        },/pgf/number format/precision=0
        ]
        coordinates {}
        [above]
        node at
        (boxplot box cs: \boxplotvalue{lower whisker},1){}
        node at
        (boxplot box cs: \boxplotvalue{lower quartile},1){}
        node at
        (boxplot box cs: \boxplotvalue{median},1){}
        node at
        (boxplot box cs: \boxplotvalue{upper quartile},1){}
        node at
        (boxplot box cs: \boxplotvalue{upper whisker},1){}
        ;
         \addplot+[black,thick,
        boxplot prepared={
            draw position=1,
            lower whisker=3.951,
            lower quartile=10.262,
            median=14.330,
            upper quartile=17.333,
            upper whisker=20.840,
        },/pgf/number format/precision=0
        ]
        coordinates {}
        [above]
        node at
        (boxplot box cs: \boxplotvalue{lower whisker},1){}
        node at
        (boxplot box cs: \boxplotvalue{lower quartile},1){}
        node at
        (boxplot box cs: \boxplotvalue{median},1){}
        node at
        (boxplot box cs: \boxplotvalue{upper quartile},1){}
        node at
        (boxplot box cs: \boxplotvalue{upper whisker},1){}
        ;
        
        \end{axis}
        \end{tikzpicture}
        \caption{{\rankdiff} of \emph{LIME} and\emph{BreakDown}} 
        \label{fig:rq4_rankdiff}
    \end{subfigure}
    \caption{Result of RQ4, comparing explanations in cross-project defect prediction scenario}
    \label{fig:rq4}
\end{figure}


==> TSE - Explainable Software Defect Prediction_ Are We There Yet_/figure/rq4n5/rq4_combine.tex <==
\begin{figure*}[t!]
\centering 
\begin{subfigure}{ 0.25\linewidth}
\centering
\includegraphics[width=\textwidth]{figure/rq4n5/rq4_cvdp_lime_hr.png}
%\vspace{-0.2in}
\caption{\small {\hitrate} of \emph{LIME}}
%\vspace{-0.1in}
\end{subfigure}\hfill
\begin{subfigure}{ 0.25\linewidth}
\centering
\includegraphics[width=\textwidth]{figure/rq4n5/rq4_cvdp_lime_rd.png}
%\vspace{-0.2in}
\caption{\small {\rd} of \emph{LIME}}
%\vspace{-0.1in}
\end{subfigure}\hfill
\begin{subfigure}{ 0.25\linewidth}
\centering
\includegraphics[width=\textwidth]{figure/rq4n5/rq4_cvdp_bd_hr.png}
%\vspace{-0.2in}
\caption{\small{ {\hitrate}} of \emph{BreakDown}}
%\vspace{-0.1in}
\end{subfigure}\hfill
\begin{subfigure}{ 0.25\linewidth}
\centering
\includegraphics[width=\textwidth]{figure/rq4n5/rq4_cvdp_bd_rd.png}
%\vspace{-0.2in}
\caption{\small{ {\rd}} of \emph{BreakDown}}
%\vspace{-0.1in}
\end{subfigure}\hfill

\vspace{-0.1in}
\caption{The detailed distributions of {\hitrate} and {\rd} of \emph{LIME} and \emph{BreakDown} on each project under the cross-version defect prediction scenario.}
\label{fig:rq4_comb}
%\vspace{-0.1in}
\end{figure*}
\vspace{-0.1in}


==> TSE - Explainable Software Defect Prediction_ Are We There Yet_/figure/rq4n5/rq5_combine.tex <==
\begin{figure*}[t!]

\centering 
\begin{subfigure}{ 0.25\linewidth}
\centering
\includegraphics[width=\textwidth]{figure/rq4n5/rq5_cpdp_lime_hr.png}
%\vspace{-0.2in}
\caption{\small {\hitrate} of \emph{LIME}}
%\vspace{-0.1in}
\end{subfigure}\hfill
\begin{subfigure}{ 0.25\linewidth}
\centering
\includegraphics[width=\textwidth]{figure/rq4n5/rq5_cpdp_lime_rd.png}
%\vspace{-0.2in}
\caption{\small {\rd} of \emph{LIME}}
%\vspace{-0.1in}
\end{subfigure}\hfill
\begin{subfigure}{ 0.25\linewidth}
\centering
\includegraphics[width=\textwidth]{figure/rq4n5/rq5_cpdp_bd_hr.png}
%\vspace{-0.2in}
\caption{\small{ {\hitrate}} of \emph{BreakDown}}
%\vspace{-0.1in}
\end{subfigure}\hfill
\begin{subfigure}{ 0.25\linewidth}
\centering
\includegraphics[width=\textwidth]{figure/rq4n5/rq5_cpdp_bd_rd.png}
%\vspace{-0.2in}
\caption{\small{ {\rd}} of \emph{BreakDown}}
%\vspace{-0.1in}
\end{subfigure}\hfill

%\vspace{-0.1in}
\caption{
% \song{jiho: need to be updated}
%\jiho{UPDATED}
The detailed distributions of {\hitrate} and {\rd} of \emph{LIME} and \emph{BreakDown} on each project under the cross-project defect prediction scenario.}
\label{fig:rq5_comb}
\end{figure*}
\vspace{-0.1in}


==> TSE - Explainable Software Defect Prediction_ Are We There Yet_/figure/rq_concept.tex <==
\begin{figure*}
     \centering
         \includegraphics[width=\textwidth]{figure/rq_concept.png}
         \caption{Overall figure of this study}
         \label{fig:rq_concept}
\end{figure*}

==> TSE - Explainable Software Defect Prediction_ Are We There Yet_/macros.tex <==
\usepackage{soul}
%\usepackage{times}
%\usepackage[T1]{fontenc}
%\usepackage{lmodern}
\usepackage{hyperref}
\usepackage{multirow}
\usepackage{listings}
\usepackage{fancybox}
\usepackage{enumitem}
\usepackage{graphicx}
%\usepackage{paralist}
%\usepackage{framed}
%\usepackage{multicols}
\usepackage{color}
\usepackage{xcolor}
\usepackage{array}
\usepackage{amsmath}
\usepackage{xspace}
\usepackage{url}
\usepackage{tikz}
\usepackage{caption}
\usepackage{pgfplots}
\pgfplotsset{compat=1.16}
\usepackage{pgf-pie}
%\usepackage[usenames,dvipsnames]{xcolor}
\usetikzlibrary{pgfplots.statistics,calc}
\usepackage{algorithm}
\usepackage{algorithmic}

\clubpenalty=100000000 %10000
\widowpenalty=10000000 %10000
\brokenpenalty=10000000 %10000

\usepackage{tcolorbox}
\makeatletter
\newcommand{\mybox}[1]{%
	\setbox0=\hbox{#1}%
	\setlength{\@tempdima}{\dimexpr\wd0+13pt}%
	\begin{tcolorbox}[boxrule=0.5pt, colback=white, arc=4pt,
		left=6pt,right=6pt,top=6pt,bottom=6pt,boxsep=0pt]
		#1
	\end{tcolorbox}
}

%
\newcommand{\tikzcircle}[2][red,fill=red]{\tikz[baseline=-0.5ex]\draw[#1,radius=#2] (0,0) circle ;}%

\definecolor{songcolor}{RGB}{191,191,191}
\newcommand{\todoc}[2]{{\textcolor{#1}{\textbf{#2}}}}
% todo commands:
\newcommand{\todored}[1]{\todoc{red}{\textbf{[[#1]]}}}
\newcommand{\todogreen}[1]{\todoc{green}{\textbf{[[#1]]}}}
\newcommand{\todoblue}[1]{\todoc{blue}{\textbf{[[#1]]}}}
\newcommand{\todogray}[1]{\todoc{Gray}{\textbf{[[#1]]}}}
\newcommand{\todoorange}[1]{\todoc{orange}{\textbf{[[#1]]}}}
\newcommand{\todobrown}[1]{\todoc{brown}{\textbf{[[#1]]}}}
\newcommand{\todopurple}[1]{\todoc{purple}{\textbf{[[#1]]}}}
\newcommand{\todoamber}[1]{\todoc{teal}{\textbf{[[#1]]}}}
%
%\newcommand{\tikzcircle}[2][red,fill=red]{\tikz[baseline=-0.5ex]\draw[#1,radius=#2] (0,0) circle ;}%


\newcommand{\add}[1]{\todored{#1}}
\newcommand{\reem}[1]{\todobrown{Reem: #1}}
\newcommand{\jiho}[1]{\todoorange{Jiho: #1}}
\newcommand{\song}[1]{\todored{Song: #1}}
\newcommand{\nima}[1]{\todoamber{Nima: #1}}
\newcommand{\jc}[1]{\todobrown{JC: #1}}
\newcommand{\jie}[1]{\todoblue{Jie: #1}}
\newcommand{\todo}[1]{\todogreen{TODO: #1}}

% --- for revision
\newcommand{\rev}[1]{\textcolor{purple}{\st{#1}}}
%\newcommand{\rev}[1]{}   
%\newcommand{\add}[1]{{#1}}
\newcommand{\tool}{\texttt{ConBP}}
\newcommand{\bugbuilding}{\texttt{ConBuild}}
\newcommand{\bugupdate}{\texttt{ConUpdate}}
\newcommand{\bugevaluate}{\texttt{ConEA}}
%% space in some tables.  BUT have it here, such that you can always renew it
\newcommand{\ts}{$\;$}
\newcommand{\tS}{$\;$}
\newcommand{\tts}{\ \ \ \ \ }
\newcommand{\tss}{\ \ \ $\;$}
\newcommand{\ttts}{$\;$}
\newcommand{\decentHLine}{\noalign{\hrule height 1.04pt}}

\newcommand{\rd}{$rank\_di\!f\!\!f\!$}
\newcommand{\rankdiff}{$rank\_di\!f\!\!f\!$}
\newcommand{\Rankdiff}{$rank\_di\!f\!\!f\!$}
%\newcommand{\rankdiff}{$ranking\_di\!f\!\!f\!erence$}
%\newcommand{\Rankdiff}{$Ranking\_di\!f\!\!f\!erence$}
\newcommand{\hitrate}{$hit\_rate$}



==> TSE - Explainable Software Defect Prediction_ Are We There Yet_/sec/abstract.tex <==
Explaining the results of defect prediction models is practical but challenging to achieve. %\nima{we have two "prediction" in one sentence} %challenging while practical task, 
%which can provide useful information for developers to understand and fix the predicted bugs. %\jc{while phrase seems having grammar error.  how about just something like is practical but challenging to achieve,`
Recently, Jiarpakdee et al. \cite{jiarpakdee2020empirical} proposed to use {two state-of-the-art} model-agnostic techniques (i.e., \emph{LIME} and \emph{BreakDown}) to explain prediction results. 
Their study showed that model-agnostic techniques can achieve remarkable performance, and the generated explanations can assist developers to understand the prediction results. 
However, the fact that they only examined both \emph{LIME} and \emph{BreakDown} in a single defect prediction setting calls into question the consistency and reliability of model-agnostic techniques on defect prediction models under various settings.

In this paper, we set out to investigate the reliability and stability of explanation generation approaches based on model-agnostic techniques, i.e., \emph{LIME} and \emph{BreakDown}, on defect prediction models under different settings, e.g., data sampling techniques, machine learning classifiers, and prediction scenarios used when building defect prediction models. 
Specifically, we use both \emph{LIME} and \emph{BreakDown} to generate explanations for the same instance under various defect prediction models with different settings and then check the consistency of the generated explanations for the instance. 
{We reused the same 
% \song{Jiho: fill here xx} 
defect data from Jiarpakdee et al. in our experiments.} 
% We reused the
% % \song{Jiho: fill here xx} 
% defect data from Jiarpakdee et al. for our experiments 
The results show that both \emph{LIME} and \emph{BreakDown} generate inconsistent explanations under different defect prediction settings for the same test instances. These imply that the model-agnostic techniques are unreliable for practical explanation generation. {In addition, our manual analysis shows that none of the generated explanations can reflect the root causes of the predicted defects, which further weakens the usefulness of model-agnostic based explanation generation.}
Overall, with this study, we {urge a revisit of existing model-agnostic based studies in software engineering} and call for more research in explainable defect prediction towards achieving reliable and stable explanation generation. 
% \song{abstract updated}
% \song{Jiho: please do not remove comments, you can comment out the ones you have addressed}
% \jiho{got it!}

==> TSE - Explainable Software Defect Prediction_ Are We There Yet_/sec/approach.tex <==
\section{Empirical Study Setup}
\label{sec:approach}


==> TSE - Explainable Software Defect Prediction_ Are We There Yet_/sec/conclusion.tex <==
\section{Conclusion}
\label{sec:conclusion}
In this paper, we investigate the reliability and stability of model-agnostic based explanation generation techniques, i.e., \emph{LIME} and \emph{BreakDown}, under different software defect prediction settings. 
Our experiments on 32 versions of defect prediction data from nine open-source projects show that neither \emph{LIME} nor \emph{BreakDown} can generate consistent explanations under different defect prediction settings, thus both are unreliable to be used in practice. 
{In addition, our manual analysis confirms that none of the generated explanations can reflect the root causes of the predicted defects.} 
Thus, {contrary to the claim of Jiarpakdee et al.~\cite{jiarpakdee2020empirical}, our study suggests % }
that model-agnostic techniques
are neither reliable nor stable to be used for explanation generation for defect prediction.} 

In the future, we plan to examine the reliability and stability of model-agnostic techniques used in other software engineering tasks and explore more reliable explanation generation techniques for prediction tasks in the software engineering domain. 


%Our experiments on 32 versions defect prediction data from nine open source projects. 
%Our analysis shows that, the explanations generated by \emph{LIME} and \emph{BreakDown} are not reasonable to be used in defect prediction scenarios. 
%Overall, with this study, we call for more research in explainable software defect prediction towards achieving consistent explanation generation.
 %comparing five data sampling techniques, six machine learning classifiers, and two defect prediction scenarios (i.e. cross-version and cross-project), we have concluded that explanations generated from these model-agnostic techniques are unreliable. 
%This is an important finding as more and more studies use model-agnostic techniques to generate explainable and actionable messages to assist developers in their debugging activities.
%It is also valid to verify the reliability of model-agnostic techniques under various different settings as there is a no cure-all technique and these tunings are widely used to mitigate other challenges, e.g. class imbalance problem and cold-start problem. 
%Therefore, we urge studies that mitigate these challenges of consistency should be in priority in applying them for actionable defect prediction. 

==> TSE - Explainable Software Defect Prediction_ Are We There Yet_/sec/contribution.tex <==
\section{*Contribution of Team Members}
\label{sec:contr}
%The contributions of each team member in our project are as following:
\vspace{4pt}
\paragraph{Tasks of Song}
\textbf{Paper Writing}: Abstract, Introduction, Background, Approach, Experiments Setup (4.1),
and Threats. 

\textbf{Project Development}: Craft the idea, Perform defect prediction and static bug finders, 
Implement QATCP algorithm, and Analyze results. 

\vspace{4pt}
\paragraph{Tasks of Yuefei}
\textbf{Paper Writing}: Related Work, Experiments Setup (4.2, 4.3, and 4.4), Results, and Conclusion. 

\textbf{Project Development}: Collect data (i.e., experiment subjects that contain real-world fault, regression fault, and mutation fault), 
Implement benchmark test case prioritization algorithms (i.e., static and dynamic coverage based, similarity based), 
Conduct experiments. 


==> TSE - Explainable Software Defect Prediction_ Are We There Yet_/sec/discussion.tex <==
\section{Discussion}
\label{sec:discussion}

\subsection{Impact of Top-N Features Used in LIME and BreakDown}
\label{sec:dis_issue1}
%\jiho{Newly Added this part, Table updated with all results combined.}
%\jiho{LIME use all the features to generate explanations but needs top-n features to show the results.
%However, the {\hitrate} and {\rd} we use to evaluate the consistency of generated explanations are affected by the size of top-n}
%Different from \emph{BreakDown}, \emph{LIME} selects the top $N$ features to generate the explanations.
Following Jiarpakdee et al.~\cite{jiarpakdee2020empirical}, in our experiments, we use top 10 features to generate explanations. However, as both the {\hitrate} and {\rankdiff} can be affected by the number of features used (i.e., $N$), we further investigate whether our findings of \emph{LIME} and \emph{BreakDown} hold when different numbers of features are used. 

For our analysis, we take our RQ1 (Section~\ref{sec:answer_rq2}) as an example to show the impact of different N on the performance of \emph{LIME} and \emph{BreakDown}. 
We follow the same process as described in Section~\ref{sec:answer_rq2} to conduct the experiments with different values of $N$. We experiment $N$ with four values, i.e., 5, 8, 10, and 15. 
For each project, we combine each of the six examined machine learning classifiers (Section~\ref{sec:classifiers}) with each of the five data sampling techniques (Section~\ref{sec:sampling}), in total, there are 30 runs, we use the two tools to generate the explanations for models before and after applying a data sampling technique and further calculate the {\hitrate} and {\rankdiff} values, finally, we average all the {\hitrate} and {\rankdiff} values on each project for each of the two examined model agnostic tools. 
Table~\ref{tab:diff_ks} shows the average {\hitrate} and {\rankdiff} of \emph{LIME} and \emph{BreakDown} with different numbers of top-N features. 
Figure~\ref{fig:diff_n} shows the detailed distribution of {\hitrate} and {\rankdiff} under a different number of top-N features.

%the different result when different top-N are used, we have calculated results with different top-N.
%Table~\ref{tab:diff_ks} shows the average {\hitrate} and {\rankdiff} of projects when using \emph{LIME} with different number of top-N features. 
%We used 5, 8, 10 and 15 to investigate the different results.
As shown in Table~\ref{tab:diff_ks}, overall, with the increase of $N$, both the {\hitrate} and {\rd} increase, this is natural because increasing $N$ will enlarge the search space of \emph{LIME} and \emph{BreakDown}, thus more matches will occur.  %when all features are used, {\hitrate} reaches the max value, i.e., 1. While with the increase of $N$, {\rd} reaches the peak when $N$ is 15 after that {\rd} decreases. The reason for this is with the number of features used, the {\rd} caused by feature missing is lower.
%For \emph{LIME}, when $N$ is 5, the {\hitrate} ranges from 0.417 to 0.494, which indicates around 3 out of \emph{LIME}'s 5 features used to generate explanations are different. 
We can see that when $N$ equals to 5, 8, 10, and 15, around 48\%, 43\%, 39\%, and 29\% features in the generated explanations of \emph{LIME} and 35\%, 31\%, 29\%, and 22\% of \emph{BreakDown} are different.  
We have also revisited other three RQs (RQ2-RQ4) by using \emph{LIME} and \emph{BreakDown} with different $N$ and we observe similar results, which indicates \emph{LIME} and \emph{BreakDown} always generates inconsistent explanations regardless of the setting of $N$.

% \song{jiho: 5.1 done, please check}
%The results indicate that when using lower value of N, the {\hitrate} gets lower and so does the {\rd}, and if N is set to a higher value, both {\hitrate} and {\rankdiff} gets higher.
%This result is natural because when fewer number of features are considered for generation explanation, the {\hitrate} will be relatively lower because it is a more difficult condition to hit.
%However the {\rankdiff} is also lower because the maximum {\rankdiff} is the same as number of N which is when a feature is not hit.


\subsection{Consistency Between the Explanations and the Root Causes of Predicted Bugs}
\label{sec:dis_issue2}

Jiarpakdee et al.~\cite{jiarpakdee2020empirical} used a set of ranked features as the explanation for a prediction. Their human-involved case study showed that 65\% of the participants agree that model-agnostic techniques can generate the time-contrast explanation to answer the why-questions like \textit{Why was file A not classified as defective
in version 1.2 but was subsequently classified as defective in version 1.3?}. 
However, it's still unknown whether the explanations are consistent with the root causes of the buggy instances. To do so, we use the LR-based defect prediction model from Jiarpakdee et al.~\cite{jiarpakdee2020empirical} to predict buggy files on the latest version of each project, we then randomly select 10 correctly predicted buggy instances from each project, in total 90 instances and their explanations generated by both \emph{LIME} and \emph{Breakdown} are collected. For each instance, we trace the data labelling process used in Jiarpakdee et al.~\cite{jiarpakdee2020empirical} to find the linked bug report(s) and we use both a report's content and its corresponding patch(es) to summarize its root cause. 
Finally, we manually (independently by the authors) check whether the generated explanations from \emph{LIME} and \emph{Breakdown} are consistent. 

Our manual analysis shows that none of the explanations generated by these tools can reflect the ground truth root causes of the predicted buggy instances. 
For example, the file ``\textit{ActiveMQConnection.java}'' showed in Figure~\ref{fig:motiv_ex} was labelled as buggy because of two bug reports, i.e., \textit{AMQ-1758}\footnote{https://issues.apache.org/jira/browse/AMQ-1758} and \textit{AMQ-1646}\footnote{https://issues.apache.org/jira/browse/AMQ-1646}, which are caused by an incorrect variable usage and an incorrect condition respectively. 
However, as shown in Figure~\ref{fig:motiv_ex}, the generated explanations are the ordered features and their numerical values, which are unrelated to the root causes, e.g., logic errors, missing API usages, syntax errors, functional errors, etc. 
%\jie{I think the results of Sec 4.1 to Sec 4.4 are quite similar, maybe we can cut these sections more or less. However, i find the findings of this sec may attracting the readers. So can we use two or three examples here. also maybe we can put the examples in a figure or table to make them more clear and attractive.}

This result is natural and expected because features used in Jiarpakdee et al.~\cite{jiarpakdee2020empirical} are all high-level software metrics, which can only capture the overall statistical characteristics of software programs. Our analysis confirms with these features, both \emph{LIME} and \emph{Breakdown} cannot generate explanations that can reflect the root causes of buggy instances, which is unreliable to be used in practice. 

%Reem~\cite{aleithan2021explainable},  manually  evaluating  the  explanationsfor  buggy  instances  (i.e.  positive  predictions)  against  the  rootcause of the bugs. The results of our experiment show that LIMEand  iBreakDown  fail  to  explain  defect  prediction  explanationsfor  just-in-time  bug  prediction  models,


\subsection{Threats to Validity}
\label{sec:threats}
\noindent \textbf{Internal Validity.} 
% \jiho{Internal validity is the extent to which a piece of evidence supports a claim about cause and effect, within the context of a particular study. It is one of the most important properties of scientific studies, and is an important concept in reasoning about evidence more generally. Internal validity is determined by how well a study can rule out alternative explanations for its findings (usually, sources of systematic error or 'bias'). It contrasts with external validity, the extent to which results can justify conclusions about other contexts (that is, the extent to which results can be generalized).}
The main internal threat of our study is the limited number of model-agnostic techniques (i.e. \emph{LIME} and \emph{BreakDown}) that we explored. Due to this limitation, we can't generalize our results to all model-agnostic techniques in the file-level defect prediction discipline. 
However, in our future studies, we will explore more techniques and compare the results to \emph{LIME} and \emph{BreakDown}. Furthermore, in this paper, we described a detailed methodology and setup of the experiment and the data set used, allowing other researchers to contribute to our study or further explore the other unexplored techniques. 


\noindent \textbf{External Validity.} 
% \jiho{External validity is the validity of applying the conclusions of a scientific study outside the context of that study. In other words, it is the extent to which the results of a study can be generalized to and across other situations, people, stimuli, and times. In contrast, internal validity is the validity of conclusions drawn within the context of a particular study. Because general conclusions are almost always a goal in research, external validity is an important property of any study. Mathematical analysis of external validity concerns a determination of whether generalization across heterogeneous populations is feasible, and devising statistical and computational methods that produce valid generalizations.}
Even though the data sets used in this work are well labelled based on ground truths, the number of the data sets is limited and makes it hard to generalize our results on other data sets and domains. Future work needs to further investigate the study on other data sets. Besides, all the experiment projects are Java projects, although they are popular projects and widely used in existing software bug prediction studies, our findings may not be generalizable to commercial projects.

% \todo{do we need this below?}
% Another limitation of the study is the number of survey participants. Our study is based on \cite{} where they only surveyed 20 software practitioners from Amazon Mechanical
% Turk. Hence, this limited sample size is not well representative of the overall software engineering practitioners population. Future work needs to further investigate a larger number of practitioners, working in different companies, in a replica of the survey.  

\noindent \textbf{Construct Validity.} 
% \jiho{Construct validity is "the degree to which a test measures what it claims, or purports, to be measuring." Is the test constructed in a way that it successfully tests what it claims to test?.}
%Construct validity is asking whether the test measures we used claim or purport what we really try to measure.
To measure the consistency of explanations generated by the same model agnostic technique (i.e., \emph{LIME} and \emph{BreakDown}) under different defect prediction settings, %generating explanations of predictions, 
%we compared the ranking of generated explanations of the baseline and each target model.
%When comparing the rankings, 
we use top 10 features in the explanations to calculate metrics {\hitrate} and {\rankdiff} following Jiarpakdee et al.~\cite{jiarpakdee2020empirical}. %In this work, we following %Basically, 
%{\hitrate} measures the situation of overlaps of features in from different explanations. %features from target models that also appears in top-ranked features from the baseline model, 
%while {\rankdiff} measures the absolute rank difference of each feature in two different explanations. % of baseline and the target models. 
%These evaluation metrics are very much related to the total number of top-ranked features selected in the beginning.
%While \emph{BreakDown} uses all the features to generate explanation (which means number of top-ranked features are 65), \emph{LIME} is set to top-10 ranked features.
With different number of features used, the {\hitrate} and {\rankdiff} of two explanations can be different, which could affect our findings. However, as we shown in Section~\ref{sec:dis_issue1}, \emph{LIME} and \emph{BreakDown} ways generates inconsistent explanations regardless of the number of features used.
%\vspace{-0.1in}
% \song{jiho:all section 5.x are done, please check}
%In We only reported the result of top-10 features because it already clearly shows that the generated explanations are very different even with small amount of rankings are considered.

% We used 10-fold cross validation techniques for RQ1-2.


==> TSE - Explainable Software Defect Prediction_ Are We There Yet_/sec/introduction.tex <==
\section{Introduction}
\label{sec:intro}
Software Defect Prediction (SDP) models have been actively studied to allocate testing resources efficiently to reduce development costs.
Most existing SDP models use various code and development metrics as features to classify a target code fragment as buggy or not. 
However, a major issue that SDP models face is that they lack actionable messages for the developers to act upon~\cite{lewis2013does}, making it very difficult for practical usage.

To address this issue, studies investigating explainable artificial intelligence (XAI) in the domain of defect prediction have been explored recently~\cite{humphreys2019explainable, 9193975, khanan2020jitbot, JiarpakdeeTG21, pornprasit2021jitline} but most of these approaches target at global explanation, which summarizes a prediction of a whole model (i.e., the relationship between defect prediction features and the bug proneness). 
%\add{For example, ... .}\jc{I think explaining some representative example approaches in this separate paragraph can be better.}
Since the global explanation does not provide a detailed interpretation of prediction results, Jiarpakdee et al.~\cite{jiarpakdee2020empirical} proposed to use the model-agnostic methods, i.e.,  \emph{LIME}~\cite{ribeiro2016should} and \emph{BreakDown}~\cite{gosiewska2019ibreakdown, staniak2018explanations} to generate instance explanation to explain the prediction of each target code fragment. 
%\rev{, i.e.,  the explanation of a prediction of a target code fragment.} 
The explanation is defined as a list of ordered features.  
%A global explanation summarizes a prediction of a whole model while instance explanation explains the prediction of each instance.
%Their primary goal was to answer the question; \textit{``Should model-agnostic techniques be used to explain the predictions of defect models?''}
Their experiments and use case studies showed that both \emph{LIME} and \emph{BreakDown} achieve promising performance and the generated explanations can assist developers by showing actionable guidance for practical usages.

However, in Jiarpakdee et al.~\cite{jiarpakdee2020empirical}, \emph{LIME} and \emph{BreakDown} were only examined on a single software defect prediction setting which leaves unanswered the more directly relevant question:
%calls into question about their consistency and reliability across software defect prediction models with various settings. 
\textit{Are model-agnostic techniques reliable and stable under defect prediction models with different settings?} 
The answer to this question is critical.
{First, many studies conduct defect prediction under different settings.
The explanations generated of model-agnostic techniques are expected to be consistent across different settings to make them reliable and stable.}
%with these method applied should be consistent as well. 
{Second, we have seen many studies follow Jiarpakdee et al.~\cite{jiarpakdee2020empirical} to use model-agnostic techniques for other tasks, e.g., defective line prediction~\cite{wattanakriengkrai2020predicting}, online buggy commit prediction~\cite{pornprasit2021jitline}, and software quality assurance planning~\cite{rajapaksha2021sqaplanner}, understanding the reliability and stability of model-agnostic techniques will help confirm the findings from inline studies and benefit future research.}

In this study, we investigate the reliability and stability of model-agnostic techniques (i.e., \emph{LIME} and \emph{BreakDown}) on software defect prediction models under different settings. 
Specifically, we consider three different settings when building software defect prediction models, i.e., data sampling techniques, machine learning classifiers, and prediction scenarios.  
Data sampling techniques are used in software defect prediction studies~\cite{wang2016automatically,tan2015online,jiang2013personalized} to solve the data imbalance issue.
In this work, we experiment with five widely used sampling methods (details are in Section~\ref{sec:sampling}). 
Various machine learning classifiers, e.g., Logistic Regression (LR), Decision Tree (DT), and Random Forest (RF), etc., have been used to build defect prediction models~\cite{kamei2012large, lessmann2008benchmarking, gao2016software, zimmermann2009cross}. 
% \song{jiho: list several citation here}
In this work, we experiment with {six} common machine learning classifiers (details are in Section~\ref{sec:classifiers}). 
Defect prediction includes two major scenarios, i.e., cross-version and cross-project defect prediction, in both scenarios, one can choose different versions of historical data to build the models.
In this work, we also examine the reliability and stability of \emph{LIME} and \emph{BreakDown} on these two scenarios when using different versions of data to build the defect prediction model. 
%Note that, in Jiarpakdee et al.~\cite{jiarpakdee2020empirical}, only a LR-based within-project software defect prediction model (without data sampling) was examined.

For our analysis, we reuse the same dataset from Jiarpakdee et al.~\cite{jiarpakdee2020empirical}, which contains 32 versions of defect data from nine large-scale open-source Java projects.
We run both \emph{LIME} and \emph{BreakDown} to generate explanations for the same instances under defect prediction models with different settings and then check the consistency of the generated explanations for the instances. 
%We conduct our experiment on 32
% \song{Jiho: fill here xx} 
%versions defect data from Jiarpakdee et al.~\cite{jiarpakdee2020empirical}'s work and the results show that both \emph{LIME} and \emph{BreakDown} generate significantly different explanations under different software defect prediction settings for the same instance. Overall, with this study, we call for more research in explainable software defect prediction towards achieving consistent explanation generation.
%However, further experiments are needed to validate the reliability of generated explanations in various settings, e.g., different data sampling techniques, different machine learning classifiers, and different prediction scenarios. 
%In Jiarpakdee et al.~\cite{jiarpakdee2020empirical}, it is difficult to say that they tested enough experiments to conclude that explanations generated from \emph{LIME} and \emph{BreakDown} is reliable. 
%This is important because plethora of studies been conducted to enhance the performance of defect prediction model and the explanations generated from models with these method applied should be consistent as well.
%To validate the reliability of generated explanations under various settings, we compare how much the generated explanations from the baseline and target models are different.
Our experimental results show that explanations generated by both \emph{LIME} and \emph{BreakDown} are significantly inconsistent when different settings are applied, {which makes them unreliable to be used in practice.
In addition, our manual analysis shows that none of the generated explanations can reflect the root causes of the predicted defects, which further weakens the usefulness of model-agnostic based explanation generation.} 
%\jc{I got the following questions: why they should be consistent? Although there is inconsistency, could the  both different messages be actionable ones? One message is invalid? is inconsistency same as conflicting explanations or could 
%complements each other?}\song{goode question, can we say: inconsistent explanations can confuse users and make the tools unreliable and impractical} 
%\jie{Actually, i have the same concern with JC. so maybe we need more clarification about this aspect. Maybe use references to back up this point. Also we can emphasize that these generated explanations are not the case of actual practices (sec 5.2)}
Hence, {contrary to the claim of Jiarpakdee et al.~\cite{jiarpakdee2020empirical}, our study suggests % }
that model-agnostic techniques %explanations generated by \emph{LIME} and \emph{BreakDown} 
are neither reliable nor stable to be used for explanation generation for defect prediction.} 
Overall, with this study, {we urge to revisit of other explainable software analytics studies that adopt model-agnostic techniques} and call for more research in explainable software defect prediction towards achieving consistent explanation generation.

This paper makes the following contributions:

\begin{itemize}
\item We perform the first study to analyze the reliability and stability of state-of-the-art model-agnostic based explanation generation techniques, i.e., \emph{LIME} and \emph{BreakDown} on software defect prediction. 

\item We examine the consistency of explanations generated by \emph{LIME} and \emph{BreakDown} under software defect prediction models with three typical settings, i.e., data sampling techniques, machine learning classifiers, and prediction scenarios.

\item We show neither \emph{LIME} nor \emph{BreakDown} can generate consistent explanations and the generated explanations cannot reflect the root causes of the predicted defects.
This makes model-agnostic techniques neither reliable nor stable to be used in practice.
Thus, we {urge a revisit of existing model-agnostic based studies in software engineering} and call for more research in building reliable and stable explanation generation for software analytics. 

\item We release the source code and the dataset of this work to help other researchers replicate and extend our study\footnote{https://doi.org/10.5281/zenodo.5425868}. 
% \song{Jiho: please create a zenodo repo and upload all you data anonymously}\jiho{all data includes all the source code as well, right?}\song{yes, code and data}
%We investigate the results of generated explanation using \emph{LIME} and \emph{BreakDown} with applying various data sampling techniques, machine learning classifiers, and different prediction scenarios.
%\item We quantitatively compare and analyze the results of generated explanation of models with or without applying aforementioned techniques.
%\item Maybe suggest other ideas ...?
\end{itemize}

We organized the rest of this paper as follows.
Section~\ref{sec:bm} presents
the background and motivation of this study. 
% Section~\ref{sec:approach} describes the
% methodology of our approach. 
Section~\ref{sec:experiment} shows the experimental setup. 
Section~\ref{sec:result} presents the evaluation results. 
Section~\ref{sec:discussion} discusses open questions and the threats to the validity of this work. 
Section~\ref{sec:related} presents the related studies. 
Section~\ref{sec:conclusion} concludes this paper. 

% \song{Jiho: Intro updated, please check}








==> TSE - Explainable Software Defect Prediction_ Are We There Yet_/sec/motivation.tex <==
\section{Background and Motivation}
\label{sec:bm}

This section introduces the background of software defect prediction models and the explanation generation techniques studied in this work and our motivation example. 

\subsection{File-level Defect Prediction Models}
\label{sec:dbmodel}
%Figure~\ref{fig:dbexample} presents 
The objective of a file-level defect prediction model is to determine risky files for further software quality assurance activities. 
~\cite{hassan09icse,zimmermann2007predicting,rahman2013and,lee2011micro,moser2008comparative,kim2007predicting,nam2013transfer}. 
A typical release-based file-level defect prediction 
model mainly has three steps. 
The first step is to label the files in an early version as buggy or clean based on post-release defects for each file.  
Post-release defects are defined as defects that are revealed within a post-release window period (e.g., six months)~\cite{rahman2013and,yan2017file}.
One could collect these post-release defects from a Bug Tracking System 
(BTS) via linking bug reports to its bug-fixing changes. 
Files related to these bug-fixing changes are considered buggy.
Otherwise, the files are labeled as clean. 
The second step is to collect the corresponding defect features to represent these files.  
Instances with features and labels are used to train machine learning classifiers. 
Finally, trained models are used to predict files in a later version as buggy or clean. 

Following Jiarpakdee et al.~\cite{jiarpakdee2020empirical}, this paper also focuses on file-level defect prediction.
%In this work, %we build bug prediction models on an early history version
%we refer to the release version used for building models as a training version, whereas the release version used to evaluate the trained models is referred to as a test version.  
\input{figure/motivation}
\subsection{Model-agnostic based Explanation Generation Techniques}
\label{sec:expTech}
Model-agnostic techniques were originally introduced to explain the prediction of black-box AI/ML algorithms by identifying the contribution that each metric has on the prediction of an instance according to a trained model~\cite{ribeiro2016model}. 
\emph{LIME}~\cite{ribeiro2016should} and \emph{BreakDown}~\cite{gosiewska2019ibreakdown, staniak2018explanations} are two state-of-the-art model-agnostic explanation techniques.

\emph{LIME}~\cite{ribeiro2016should} mimics a black-box model it aims to explain.
To generate an explanation of an instance, \emph{LIME} follows four major steps.
It first creates synthetic instances around the instance to be explained.
Then, it generates predictions of all the synthetic instances generated in the step above.
After that, it creates a local regression model with the synthetic instances and their predictions made in the step above.
Finally, using the regression model, \emph{LIME} ranks the contribution of each metric to the predictions aligning with the black-box model. 
\emph{BreakDown}~\cite{gosiewska2019ibreakdown, staniak2018explanations} measures the additive contribution of each feature of an instance sequentially, summing up to the final black-box prediction result. 
In our study, we used the ag-break version of the \emph{BreakDown} technique, which works for non-additive models following Jiarpakdee et al.~\cite{jiarpakdee2020empirical}.
%\emph{ag-break} aims to find features which would change the prediction significantly if they are changed.
%To be more specific, ag-break uses a greedy algorithm on the distance to relaxed model prediction to identify which set of features give the minimal distance.
%This greedy search can be done in two different ways: \textit{step-up} and \textit{step-down}.
%The \textit{step-down} approach starts with the entire set of features and greedily selects features with small distance to relaxed model predictions.
%While the \textit{step-up} approach does the same methodology but selecting the features with the large distance to relaxed model predictions instead \cite{staniak2018explanations}.

Jiarpakdee et al.~\cite{jiarpakdee2020empirical} are the first to leverage model-agnostic explanation techniques to generate 
instance explanations, which refer to an explanation of the prediction of defect prediction models.
The techniques define explanations as a list of ordered features. 
In this work, we empirically evaluate the reliability and stability of model-agnostic explanation techniques on software defect prediction models with different settings. 
%Since both \emph{LIME} and \emph{BreakDown} are model-agnostic, they both explain prediction instances of a black-box model.
%Some of the advantages of using these model-agnostic techniques include:
%(1) their ability to interpret any classification model (such as regression, SVM, XGBoost, and random forest);
%(2) their ability to process any type of data (e.g. tabular or images);
%and (3) their flexibility with the form explanations (e.g. rules or feature importance). 

\subsection{Motivating Example}
\label{sec:motivation}



%Jiarpakdee et al.~\cite{jiarpakdee2020empirical} used model-agnostic techniques, i.e. \emph{LIME} and \emph{BreakDown}, to explain the results of defect prediction models so that the developers can act upon.
%For practical usage, generated explanations must be reliable and stable regardless the defect prediction settings adopted. 
%the data sampling, or machine learning classifiers in different defect prediction scenarios (with-in project, cross-version, cross-project, etc.). 
In this section, we introduce an example to illustrate the problem of explanations generated by a model-agnostic technique, i.e., \emph{LIME}, which motivates us to further explore the reliability and stability of model-agnostic based explanation generation. 
%of the experiment.

Figure~\ref{fig:motiv_ex}
% \song{jiho: generated by LIME or bREAKDOWN?}
% \jiho{generated by LIME}
shows the explanations generated by \emph{LIME} for file \textit{``ActiveMQConnection.java''} with different software defect prediction models (i.e., LR in Figure~\ref{fig:motiv_ex_1} and DT in Figure~\ref{fig:motiv_ex_2}) from version 5.0.0 of project ActiveMQ. 
The figures list the ranking of features that contribute to the prediction, i.e., explanations of the prediction.
Figures on the left side are the probability and explanation of features that contribute to a prediction.
%For example, in Figure~\ref{fig:motiv_ex_1}, the file was predicted as buggy with a probability of 0.9 (i.e., sum of the probability of each selected feature) and explanation for the prediction can be summarized as: \#COMM > 3, \#coutDelMethodProtected > 10, \#MaxinheritanceTree >= 1, etc. 
On the right side, the figure depicts the actual value of the feature.
For example, in Fig.~\ref{fig:motiv_ex_1}, ``COMM'' contributes 0.39 buggy-prone because the value is 11, which is over 3.
The orange color shows that a feature contributes in predicted as buggy and blue shows it contributes in predicted as clean. 
%\song{Jiho: The value of each selected feature represents ?}
%\jiho{The value is the actual value of the features}
%Figure~\ref{fig:motiv_ex_1} has a prediction probability of 1.0 and Fig.~\ref{fig:motiv_ex_2} has a prediction probability of 0.86.\song{where you get the probability?}
%Even though the actual difference of the two models is using different machine learning classifiers, i.e. logistic regression and SVM, the generated explanation is very much different.
{Although under both software defect prediction models, the file is predicted as buggy, the generated explanations are significantly different.
Specifically, among the ten features selected by \emph{LIME}
%to explain why the file is predicted as buggy 
on the LR-based defect prediction model, only two were also selected on the DT-based defect prediction model, i.e., ``DDEV'' and ``MaxCylomatic''.
However, ``DDEV'' and ``MaxCylomatic'' have different ranks.}
With this much difference, the generated explanation is unreliable and hard to be trusted. %by the developers in using them as an actionable message.
%\jc{if we assume there is consistent results, then how the top features can be the actionable messages? Since CountLine is top ranked by DT, then the actionable message is `remove code lines'? }
%\song{I do not think it can be used to fix bugs, Jiarpakdee et al.'s use case study reported developers think the explanations generated by these tools are necessary and useful to understand the predictions of defect models. I think we can make this point clear in intro} 
% Our motivation suggests that even when researchers use different settings, i.e. feature selection, data sampling, machine learning classifiers, and prediction scenario, the generated explanation of an instance must be consistent. 

Motivated by this example, in this work we perform a comprehensive assessment and in-depth analysis of the state-of-the-art model-agnostic based explanation generation techniques, i.e., \emph{LIME} and \emph{BreakDown} on defect prediction models with different settings. {Note that the goal of this study is to evaluate the reliability and stability of a model-agnostic technique against itself under different software defect prediction models, not to evaluate one model-agnostic technique against another.}
%\emph{LIME} against \emph{BreakDown}. We

% \song{jiho: Background and Motivation updated, please check}

==> TSE - Explainable Software Defect Prediction_ Are We There Yet_/sec/related.tex <==
\section{Related Work on Explainable Defect Prediction}
\label{sec:related}
%\subsection{Explainable Defect Prediction} 
As analytical modelling advances in the software engineering domain, the lack of explainability of analytical models becomes more problematic. Recent studies show the importance and need for such explanations~\cite{radford2017learning}. Even more, as Dam et al., Lewis et al., Menzies and Zimmermann emphasize, these analytical model explanations need to be actionable to provide the most value and practical use to both practitioners and software engineers~\cite{radford2017learning, lewis2013does, 6547619,JiarpakdeeTG21}. 

Many efforts have been done to build explainable software defect prediction models~\cite{humphreys2019explainable,jiarpakdee2020empirical,khanan2020jitbot,pornprasit2021jitline,9193975,lundberg2017unified,ribeiro2018anchors}. 
%Within the context of SDP, 
Jiarpakdee et al.~\cite{JiarpakdeeTG21} conducted a qualitative survey that investigates developers' perception of defect prediction goals and their explanations. 
The results of their experiments showed that majority of the respondents believed that software defect prediction is very important and useful and  \emph{LIME} and %ranked the highest in terms of the usefulness, quality, and insightfulness of the explanations, with a 66-76 percent agreement among the respondents, as compared to other techniques in terms of its understanding of the most important characteristics contributing to a prediction of a file being defected or not; (3) 
\emph{BreakDown} are ranked as the top two approaches among a list of explanation generation approaches, in terms of the usefulness, quality, and insightfulness of the explanations. %.the %second in place also on the quality, insightfulness, and usefulness, with a 60-70 percent agreement among the respondents. 
% \begin{itemize}
%     \item explain the need and goals of model-agnostic explanations in defect prediction for practitioners including the names in the paper
%     \item explain the survey they conducted (brief methodology and metrics). 
%     \item give a little bit of statistics on the acceptance and rank of lime and breakdown among the practitioners.
%     \item (1) 82-84 percent of the respondents perceived that the three goals of defect prediction models are useful; (2) E is the most preferred technique for understanding the most important characteristics that contributed to a prediction of a file with an agreement percentage of 66-78 percent along three dimensions.
% \end{itemize}
%\subsection{Analytical Models for Explainable Defect Prediction}
Humphreys and Dam~\cite{humphreys2019explainable} proposed an explainable deep learning defect prediction model which exploits self-attention transformer encoders. By using self-attention transformer encoders, the model can disentangle long-distance dependencies and benefit from its regularizing effect.
Also, they can normalize correlations that are inversely proportional to the prediction for more useful data. Jiarpakdee et al. \cite{jiarpakdee2020empirical} used \emph{LIME} and \emph{BreakDown} to generate explanations on file-level defect prediction models that show which metrics are associated with buggy predictions. 
Khanan et al. \cite{khanan2020jitbot} proposed an explainable JIT-DP framework, \emph{JITBot}, that automatically generates feedback for developers by providing risks, and explaining the mitigation plan of each commit.
They used Random forest classifier for risk introducing commit prediction and leveraged model-agnostic technique, i.e. \emph{LIME}, to explain the prediction results. %Finally, they integrated their tools in a GitHub-based platform for continuous monitoring and analyses. 
Pornprasit and Tantithamthavorn~\cite{pornprasit2021jitline} proposed \emph{JITLine}, which ranks defective lines in a commit for finer granularity. 
With \emph{JITLine}, they are able to predict both defect-introducing commits and identify lines that are associated with the commit. They exploit Bag-of-Token features extracted from repositories and apply them on machine learning classifiers to calculate the defect density of each commit. Then, they use defect density scores to rank different lines of the commit as risky. 
Wattanakriengkrai et al. \cite{9193975} proposed a framework called \emph{LINE-DP}, which applies \emph{LIME} on a file-level prediction model trained with code token features.
The explanation generated from \emph{LIME} will show which code tokens are introducing bugs in the file.
Then they use these explanations to identify a line buggy if the line contains bug-prone tokens. 
Lundber and Lee \cite{lundberg2017unified} proposed {SHAP} which is a model-agnostic technique that works similarly to \emph{BreakDown}, however instead of using the greedy strategy, it uses game theory to calculate the contribution probability of each feature to the final prediction of the prediction model. 
Ribeiro et al. \cite{ribeiro2018anchors} proposed Anchors. \emph{Anchor} is an extension of \emph{LIME} generating rule-based explanations using decision rules. These rules are if-then rules (anchors) that have high confidence (at least 95\% confidence and highest coverage if more than one rule has the same confidence value). In other words, only the selected features by \emph{anchor} affect the final prediction. 

Recently, Reem~\cite{aleithan2021explainable} conducted the first study to manually check whether the explanations generated by \emph{LIME} and \emph{BreakDown} are the same as the root cause of the bugs for change-level defect prediction models. Their results showed that both \emph{LIME} and \emph{BreakDown} fail to explain the root causes of predicted buggy changes. 
In this work, we conduct an empirical study to analyze the reliability and stability of model-agnostic based explanation generation techniques, i.e., \emph{LIME} and \emph{BreakDown} on software defect prediction under various settings at file-level defect prediction and we have also conducted the same manual analysis as Reem~\cite{aleithan2021explainable} on file-level defect prediction models and our manual analysis confirms the same finding, i.e., both \emph{LIME} and \emph{BreakDown} fail to explain the root causes of predicted buggy instances.
% \song{jiho:  6 is done}
%\vspace{-0.2in}

==> TSE - Explainable Software Defect Prediction_ Are We There Yet_/sec/result.tex <==
\section{Results and Analysis}
\label{sec:result}
This section presents the experimental results and the answers to the research questions regarding the reliability and stability of model-agnostic techniques proposed in Section~\ref{sec:rq}.
%The result of each research questions are plotted as a box plot in Fig~\ref{fig:rq2_comb}$\sim$\ref{fig:rq5_comb}.
%The average of each results per method is organized in Table~\ref{tab:average}.
\input{table/average}

\begin{comment}
\subsection{RQ1: Explanation Consistency Under Different Feature Selection Techniques}
\label{sec:answer_rq1}
\noindent \textbf{Approach:}To investigate the consistency of the generated explanation under different feature selection approaches, we compare the hit rate and ranking difference of three different types of commonly used feature selection methods.
First, the baseline defect prediction model is built with logistic regression on data that is applied with feature selection based on Spearman's rank correlation coefficient.
Then we create \emph{LIME} and \emph{BreakDown}'s explainer on the built prediction model.
We build another model with logistic regression and the corresponding explainer on data with applying each feature selection technique.
Then we generate explanations of test instances that the models predicted as buggy to retrieve the {\hitrate} and {\rankdiff}.
In this paper, we use top\_10 features to generate explanations of \emph{LIME}.
We use 10 fold cross-validation to generate train and test set.
We report the average of each fold's calculated {\hitrate} and {\rankdiff}.

% \input{figure/rq1/rq1_combine}

\noindent \textbf{Result:} As shown in Fig.~\ref{fig:rq1_comb}, average {\hitrate} of feature selection model ranges to xx ~ xx.
Almost xx\% of the features of generated explanation is different when different feature selection method is applied.
When we look at {\rankdiff}, we can see that about X ranks are different in \emph{LIME} and X ranks are different in \emph{BreakDown}.
Considering that we used top-10 features in generating \emph{LIME}'s explanation, X rank difference can be considered high.
Also in \emph{BreakDown}, considering that there are X features in total, more than X\% of the rankings are different when other feature selection is applied.
This could be problematic because many studies apply feature selection to eliminate multicollinearity.
From these observations we can see that explanation generated by \emph{LIME} and \emph{BreakDown} is not very reliable when feature selection is applied.

\mybox{\textbf{Result of RQ1:} {\hitrate} ranges to 0.522$\sim$0.579 and {\rankdiff} is about 6 for \emph{LIME} and about 14 for \emph{BreakDown} when data sampling is applied.
This shows that \emph{LIME} and \emph{BreakDown} has low reliability in generating explanations when data sampling techniques are applied.}
\end{comment}

\input{figure/rq2/rq2_combine}
%\input{figure/rq3/rq3_combine}
\subsection{RQ1: Explanation Consistency Under Different Data Sampling Techniques}
\label{sec:answer_rq2}
\noindent \textbf{Approach:} To investigate the consistency of the generated explanations of a model-agnostic technique under different data sampling approaches, we combine the defect prediction setting (i.e., each of the classifiers listed in Section~\ref{sec:classifiers} in the within-version defect prediction scenario
%\jiho{only did LR for this RQ. Maybe you meant different data sampling techinques in Section \ref{sec:sampling}?}) 
used in Jiarpakdee et al.~\cite{jiarpakdee2020empirical} with different data sampling techniques to build defect prediction models on each experimental project. 
We follow Jiarpakdee et al. to use the out-of-sample bootstrap validation 
%\jiho{currently using 10 fold cross-validation}
technique to create the training and test data on each version of each project listed in Table~\ref{tab:expprojects}.  
On the same test dataset, we run both \emph{LIME} and \emph{BreakDown} under Jiarpakdee et al.'s defect prediction model and its variant with data sampling techniques to generate explanations for test instances that are predicted as buggy in both models. 
We use the {\hitrate} and {\rankdiff} to evaluate the consistency of explanations generated by \emph{LIME} and  \emph{BreakDown}. 
%we compare the hit rate and ranking difference of five different types of commonly used data sampling methods.
%First, the baseline defect prediction model is built with logistic regression on data without applying data sampling techniques.
%Then we create \emph{LIME} and \emph{BreakDown}'s explainer on the built prediction model.
%We build another model with logistic regression and the corresponding explainer on data with applying each data sampling techniques.
%Then we generate explanations of test instances that the baseline predicted as buggy to retrieve the {\hitrate} and {\rankdiff}.
%While \emph{BreakDown} uses all the given features to generate the explanation, \emph{LIME} takes top\_k number of features.
%In this paper, we use top\_10 features to generate explanations of \emph{LIME}.
%We use 10 fold cross-validation to generate train and test set. 
{In total, we have 60 runs on each project, i.e., 6 classifiers * 5 data sampling * 2 options (with or without sampling), for both \emph{LIME} and \emph{BreakDown}.} 
We report the average values of {\hitrate} and {\rankdiff} of explanations generated by the same model-agnostic technique under defect prediction models {with or without} different data sampling techniques applied. In this RQ, we examine two typical model-agnostic techniques, i.e.,
\emph{LIME} and \emph{BreakDown}.\vspace{4pt}

%\jc{I could not get easily what classifier was used for RQ1. Used all 6 classifiers with or without sampling techniques?}
%For \emph{BreakDown}, only {\rankdiff} is reported because \emph{BreakDown} uses all the features to explain the prediction, hence the {\hitrate} will always be 100\%.

\noindent \textbf{Result:} Table~\ref{tab:average} shows the average {\hitrate} and {\rankdiff} {of explanations generated from the same model-agnostic technique} before and after applying each data sampling technique. Figure~\ref{fig:rq2_comb} shows the detailed distribution of {\hitrate} and {\rankdiff} on each project. 
Overall, both \emph{LIME} and \emph{BreakDown} generate inconsistent explanations on defect prediction models before and after applying different data sampling techniques. 
%\jc{In section 3.1, measures are computed from two different models. This may confuse readers. I also got confused. two different models are easily perceived as LIME vs. Breakdown. However, in RQ1, a classifier with sampling vs. a classifier without sampling? right?} 
%Compared to \emph{LIME}, \emph{BreakDown} has better performance, i.e., lower {\hitrate} and {\rankdiff}. 
Specifically, the average {\hitrate} values of \emph{LIME} and \emph{BreakDown} range from 0.574 (using Random under-sampling) to 0.641 (using Random over-sampling) and 0.655 (using Cluster Centroids) to 0.769 (using Random over-sampling), respectively,
% \jie{the largest is 0.694 for Random over-sampling}
which implies almost 40\% and 29\% of the features in the generated explanations of \emph{LIME} and \emph{BreakDown} are different before and after data sampling techniques are applied. 

Regarding {\rankdiff}, on average, 5 out of the 10 features in the explanations from \emph{LIME} and 4 out of 10 features from \emph{BreakDown} have different ranks,  
%Considering that \emph{LIME}'s explanation only contains 10 top features, 
which implies on average 50\% and 40\% features in the explanations generated by \emph{LIME} and \emph{BreakDown} have a different order under defect prediction models before and after data sampling applied. 
%In \emph{BreakDown}, there are 22$\sim$27 features in total, more than 16\% features 
%{\jiho{Since breakdown uses all features, every features are present when comparing and because all features different, the highest {\rd} for breakdown is about 13.48 (See Sec. 3.6). Should we mention this part in the results? That 5 ranks are high when highest can be 13.48?}}
%have a different rank when data sampling is applied. 

In addition, we have also checked that for both \emph{LIME} and \emph{BreakDown}, {100\%} of test instances have different feature orders before and after applying data sampling techniques. 
%This could be problematic because defect prediction suffers from severe class imbalance problem.
%Therefore it is very common to apply data sampling techniques to mitigate this problem \cite{wang2013using, li2012sample, feng2021investigation}.
From these observations, we can see that explanations generated by \emph{LIME} and \emph{BreakDown} are inconsistent when data sampling is applied, which makes them unreliable and unstable.  

%\jie{It seems that a lower percentage of features have different orders in Breakdown than in Lime, are there any explanation for that? Does it because of the Breakdown consider more features? are there any other reasons? In other words, if one of the investigated approaches is better than another, maybe we can add more content to discuss them. In this current version, only the number are presented which is too straightforward, maybe more deeper discussions can be added.}
%\jiho{About the difference of {\rankdiff} of LIME and BreakDown, the original journal shows a similar result. They did a consistency test by checking if same explanations are generated when they repeat the generation by 100 times. BreakDown had \rankdiff value which converged to zero while LIME had median of seven. (they use all features on LIME)}

\mybox{Both \emph{LIME} and \emph{BreakDown} generate inconsistent explanations when data sampling is applied. On average, almost 40\% of the features in the explanations generated by \emph{LIME} and 29\% from \emph{BreakDown} are different when data sampling techniques are applied. 
In addition, around 50\% and 40\% of features in the explanations generated by \emph{LIME} and \emph{BreakDown} have different orders under any data sampling technique.}
%\mybox{$Hit\_rate$ ranges to 0.600$\sim$0.685 and {\rd} is about 5 for \emph{LIME} and about 4 for \emph{BreakDown} when data sampling is applied.This shows that \emph{LIME} and \emph{BreakDown} has low reliability in generating explanations when data sampling techniques are applied.}

% \song{jiho: 4.1 is done, please check}

\subsection{RQ2: Explanation Consistency Under Different Classifiers}
\label{sec:answer_rq3}
\noindent \textbf{Approach:} To investigate the consistency of the generated explanations of the same model-agnostic technique under defect prediction models trained on different machine learning classifiers, 
%for the same test data of \emph{LIME} and \emph{BreakDown} under different machine learning classifiers trained on the same training data, 
we use the six widely-used machine learning classifiers as our experiment subjects (details are in Section~\ref{sec:classifiers}). 
Note that, to avoid potential bias, we do not apply any data sampling technique in RQ2. 
For each classifier, we follow the process described in Jiarpakdee et al.~\cite{jiarpakdee2020empirical} to create the training and test data. We use the LR-based software defect prediction model as the baseline as suggested in~\cite{jiarpakdee2020empirical} %\jc{why LR is baseline? because of ~\cite{jiarpakdee2020empirical}?} 
for the comparison. On the same test dataset, we run a model-agnostic technique on both the baseline (LR-based defect prediction model) and each of the other five examined classifiers, i.e., DT, RF, AVNNet, GBM, and xGBTree, to generate explanations for test instances. When different machine learning models are applied, prediction results of the same instance vary as buggy or clean.
So, we only consider instances that are predicted as buggy in both compared machine learning predictors. 
To measure the consistency, we use {\hitrate} and {\rankdiff} to evaluate \emph{LIME} and  \emph{BreakDown} on different classifiers. 
We report the average values of {\hitrate} and {\rankdiff} across all the experiment projects when comparing two classifiers. In this RQ, we also examine two model-agnostic techniques, i.e., \emph{LIME} and \emph{BreakDown}. 
%of six different types of commonly used machine learning classifiers.
%Similar to section~\ref{sec:answer_rq2}, the baseline defect prediction model is built with logistic regression on data without applying data sampling techniques. 

%Then we create \emph{LIME} and \emph{BreakDown}'s explainer on the built prediction model.
%We build another model with different machine learning classifiers.
%Then we generate explanations for test instances that are predicted buggy in both models and retrieve the {\hitrate} and {\rankdiff}.

%We use 10 fold cross-validation to generate train and test set.
%We report the average of each fold's calculated {\hitrate} and {\rankdiff}.
%The result is organized in Fig.~\ref{fig:rq3_comb}.
%For \emph{BreakDown}, only {\rankdiff} is reported because \emph{BreakDown} uses all the features to explain the prediction, hence the {\hitrate} will always be 100\%.
\input{table/classifierAvg}

\vspace{4pt}

\noindent \textbf{Result:} 
Table~\ref{tab:ml_avg} shows the average {\hitrate} and {\rankdiff} of the two explanation generation tools on different machine learning classifiers. Overall, both \emph{LIME} and \emph{BreakDown} generate inconsistent explanations between different machine learning classifiers. 
For \emph{LIME}, the average {\hitrate} on these projects ranges from 0.515 (i.e., DT) to 0.613 (i.e., AVNNet), 
% \song{Jiho: fill numbers here}
which means around 44\% of the features in \emph{LIME}'s explanations are different when a different machine learning classifier is applied for defect prediction compared to LR based defect prediction model. 
\emph{BreakDown} has a slightly higher {\hitrate}, around 36\% of the features in \emph{BreakDown}'s explanations are different when different machine learning classifiers are applied. 
In addition, all the {\rankdiff} values of \emph{LIME} and \emph{BreakDown} are higher than 4 and our analysis further reveals that on average there are more than 5 and 4 features in the explanations generated by \emph{LIME} and  \emph{BreakDown} that have different ranks under software defect prediction models with different classifiers, which indicates 50\% and 40\% features in the generated explanations have different orders. 
%\jie{Can also present the percentage of different ranked features here.}
%Compared to RQ1, we can see that the generated explanations from different machine learning classifiers are more different. 
%Hence the generated explanation of \emph{LIME} and \emph{BreakDown} is not suitable for actionable message.
Note that, because of the space limitation, we only show the results of experiments whose base model is LR, we have also used each of the studied machine learning classifiers as the base model, and we observe similar findings, which indicates \emph{LIME} and \emph{BreakDown} consistently generate unreliable explanations when different classifiers are applied.

\mybox{%The explanations generated by Both 
Both \emph{LIME} and \emph{BreakDown} generate inconsistent explanations under different classifiers. %dramatically when different machine learning classifiers are used compared to LR. 
Specifically, on average, 44\%
% \song{jiho:fill here}
of the features in \emph{LIME}’s explanations and 36\% of the features in \emph{BreakDown}’s explanations are different when different machine learning classifiers are applied. 
In addition, more than 50\% and 40\% of the features in the explanations generated by \emph{LIME} and \emph{BreakDown} have different orders when different machine learning classifiers applied.} 
% \song{jiho: 4.2 done, please check}

\input{figure/rq4n5/rq4_combine}
\input{figure/rq4n5/rq5_combine}
\subsection{RQ3: Explanation Consistency Under the Cross-Version Scenario}
\label{sec:answer_rq4}

\noindent \textbf{Approach:} To investigate the consistency of the generated explanations of a model-agnostic technique under cross-version defect prediction scenario, for each experiment project listed in Table~\ref{tab:expprojects}, we use its latest version as the test data, and we then randomly select two different versions from the same project as the training data to train two different software defect prediction models.
We run the model-agnostic technique under both models to generate explanations for test instances that are predicted as buggy in both models. 
We use the {\hitrate} and {\rankdiff} to evaluate the consistency of explanations generated by the model-agnostic technique. %by \emph{LIME} and \emph{BreakDown} under different models. 
Note that, in this study, we use six different classifiers (details are in Section~\ref{sec:classifiers}) and examine two model-agnostic techniques, i.e., \emph{LIME} and \emph{BreakDown}. %\jiho{only LR for now} 
%(details are in Section~\ref{sec:classifiers}), 
%We use each classifier to run the experiments, thus each project has 6 experiment runs for examining the consistency of the generated explanations of \emph{LIME} and \emph{BreakDown} and 
%We use the average {\hitrate} and {\rankdiff} to measure the consistency of a examined model-agnostic technique. 
%we compare the hit rate and ranking difference when predicting instances from different version of a project.
%The baseline defect prediction model is built with logistic regression.
%Then we create \emph{LIME} and \emph{BreakDown}'s explainer on the built prediction model.
%We build another model with data from different version of the same project.
%Then we generate explanations of test instances that the baseline predicted as buggy to retrieve the {\hitrate} and {\rankdiff}.
%We use all the data from different version of the same project.
%We report the average of each version calculated {\hitrate} and {\rankdiff}.
%The result is organized in Fig.~\ref{fig:rq4_comb}.
%For \emph{BreakDown}, only {\rankdiff} is reported because \emph{BreakDown} uses all the features to explain the prediction, hence the {\hitrate} will always be 100\%.

\vspace{4pt}

\noindent \textbf{Result:} 
%\jiho{would a table for showing average result of RQ3\&4 be necessary?}
Table~\ref{tab:rq34} shows the average {\hitrate} and {\rankdiff} of \emph{LIME} and \emph{BreakDown} under the cross-version prediction scenario and Figure~\ref{fig:rq4_comb} shows the detailed distributions of {\hitrate} and {\rankdiff}.  
% Note that, for \emph{BreakDown}, only {\rankdiff} is reported because \emph{BreakDown} uses all the features to explain the prediction, hence the {\hitrate} will always be 100\%.
% \jie{this sentence do not necessary put here, since this is the same in all these experiments. We can put this sentence in Sec 4.1, or Sec 3.6 }
As we can see from the results, the {\hitrate} values of both \emph{LIME} and \emph{BreakDown} are higher than 0.4 on each project. 
On average, {\hitrate} is 0.518 across all the projects for \emph{LIME}, which means around 50\% of the generated explanations of \emph{LIME} are different under cross-version defect prediction. 
For \emph{BreakDown}, we can see that its average {\hitrate} is 0.591, indicating 41\% of the generated explanations are different under cross-version defect prediction. 

In addition, we can see that the {\rankdiff} of both \emph{LIME} and \emph{BreakDown} on most projects are higher than 5, which indicates around 50\% of features in the generated explanations of both \emph{LIME} and \emph{BreakDown} have different orders under defect prediction models built on different versions. 

%This could be problematic because cross-version defect prediction scenario is very practical in projects with historical data because the distribution difference will be much lower \cite{yang2018ridge, xu2018cross}.

\mybox{Both \emph{LIME} and \emph{BreakDown} generate inconsistent explanations under cross-version defect prediction scenarios. 
Overall, 50\% of features in the generated explanations of \emph{LIME} and 41\% of \emph{BreakDown} are different. In addition, around 50\% of features in the generated explanations of \emph{LIME} and \emph{BreakDown} have different orders under the cross-version defect prediction scenario.} 
%This shows that \emph{LIME} and \emph{BreakDown} has low reliability in generating explanations when different versions are used in prediction.}
% \song{jiho: 4.3 done, please check}
\input{table/RQ34}

\subsection{RQ4: Explanation Consistency Under the Cross-Project Scenario}
\label{sec:answer_rq5}

\noindent \textbf{Approach:} To investigate the consistency of the explanations generated by a model-agnostic technique under cross-project defect prediction scenario, we first randomly select one version from each experiment project as the test data, 
%\jiho{I did all versions for test data}
we then randomly select two different versions from two different projects respectively as the training data to build two defect prediction models.
We run the model-agnostic technique to generated explanations for test instances that are predicted as buggy in both models. 
We then use the {\hitrate} and {\rankdiff} to evaluate the consistency of explanations generated by the model-agnostic technique.  
In addition, we use each of the six studied classifiers to run the experiments. 
%\jiho{only LR for now}
We repeat the above process 10 times for avoiding potential data selection bias. 
Thus, each project has 6*10 experiment runs for examining the consistency of the generated explanations. 
We examine the studied two model-agnostic techniques, i.e., \emph{LIME} and \emph{BreakDown}. 
Similar to other RQs, we use the average {\hitrate} and {\rankdiff} of each run to measure the consistency. %Similar to RQ3, we only show {\rankdiff} for \emph{BreakDown}. 
%Note that, for \emph{BreakDown}, only {\rankdiff} is reported because \emph{BreakDown} uses all the features to explain the prediction, hence the {\hitrate} will always be 100\%. 
 

%we compare the hit rate and ranking difference when predicting instances from a different project.
%The baseline defect prediction model is built with logistic regression.
%Then we create \emph{LIME} and \emph{BreakDown}'s explainer on the built prediction model.
%We build another model with data from a different project.
%Then we generate explanations of test instances that the baseline predicted as buggy to retrieve the {\hitrate} and {\rankdiff}.
%We pick two random data sets from different projects as training set.
%The result is organized in Fig.~\ref{fig:rq5_comb}.
%For \emph{BreakDown}, only {\rankdiff} is reported because \emph{BreakDown} uses all the features to explain the prediction, hence the {\hitrate} will always be 100\%.

\input{figure/diff_n/diff_n}

\vspace{4pt}

\noindent \textbf{Result:} 
Table~\ref{tab:rq34} shows the average {\hitrate} and {\rankdiff} of the two explanation generation tools under the cross-project prediction scenario. 
Figure~\ref{fig:rq5_comb} presents the detailed distribution of {\hitrate} and {\rankdiff} for \emph{LIME} and \emph{BreakDown} on each project. As we can see from the figures, the average {\hitrate} of \emph{LIME} is around 0.48 on each project, which meaning around 52\% of features in the generated explanations of \emph{LIME} are different under the cross-project defect prediction scenario. 
For \emph{BreakDown}, the average {\hitrate} is 0.51, indicating 49\% features in the generated explanations are different under the cross-project defect prediction scenario. 

In addition, we can see that the {\rankdiff} values both of \emph{LIME} and \emph{BreakDown} are around 6 on each project, which indicates 60\% of features in the generated explanations of them have different orders under the cross-project defect prediction scenario.

%As shown in Table.~\ref{tab:average}, the {\hitrate} of \emph{LIME} is about 0.5, meaning about 50\% of the generated explanations from predicting with different project are different.
%Also we can see that the {\rankdiff} of \emph{LIME} averages 6 ranks and \emph{BreakDown} averages 7 ranks.
%This could be problematic because cross-project defect prediction scenario is also widely studied to mitigate cold-start problem that defect prediction models face \cite{zimmermann2009cross, he2012investigation, guo2016cold}.

\mybox{Both \emph{LIME} and \emph{BreakDown} generate inconsistent explanations under the cross-project defect prediction scenario. 
Specifically, around 52\% of the features in the generated explanations of \emph{LIME} and 49\% for \emph{BreakDown} are different under the cross-project defect prediction scenario. In addition, 60\% of features in the generated explanations have different orders.}  
%This shows that \emph{LIME} and \emph{BreakDown} has low reliability in generating explanations when different projects are used in prediction.}

% \song{jiho: 4.4 done, please check}
\input{table/discussion2}

==> TSE - Explainable Software Defect Prediction_ Are We There Yet_/sec/setup.tex <==
\section{Empirical Study Setup}
\label{sec:experiment}

This section describes our experiment method for evaluating the reliability and stability of model-agnostic based explanation generation techniques, i.e., \emph{LIME} and \emph{BreakDown}, on defect prediction models in various settings.
%Fig~\ref{fig:rq_concept} illustrates the high-level concept of our experiment.

%\input{figure/rq_concept}

\subsection{Research Questions}
\label{sec:rq}
To achieve the mentioned goal, we have designed experiments to answer the following research questions regarding the reliability and stability of each of the two studied model-agnostic based explanation generation techniques (i.e., \emph{LIME} and \emph{BreakDown}):
% \textbf{RQ1:} Are the generated explanations consistent under different feature selection methods? 
\vspace{4pt}

\noindent \textbf{RQ1:} \textit{Are the generated explanations from the same tool consistent under different data sampling techniques?} 

\vspace{4pt}

Software defect data are often imbalanced~\cite{tan2015online}, i.e., the buggy instances are much fewer than the clean ones.
Resampling, which changes the distribution between the majority class and the minority class, is an effective way to mitigate the effects of imbalanced data~\cite{wang2013using,wang2016automatically}. 
Thus, applying data sampling techniques is a common step in defect prediction~\cite{tan2015online}.
However, in Jiarpakdee et al.~\cite{jiarpakdee2020empirical}, no data sampling techniques were applied. 
In RQ1, we investigate whether a model-agnostic technique based explanation tool can generate consistent explanations for the predicted buggy instances under the software defect prediction model with applied different data sampling techniques. 

\vspace{4pt}
\noindent \textbf{RQ2:} \textit{Are the generated explanations from the same tool consistent under different machine learning classifiers?}  

\vspace{4pt}

To build accurate software defect prediction models, different machine learning classifiers have been used to build software defect prediction models, e.g., Logistic Regression (LR), Decision Tree (DT), Random Forest (RF), etc.
Researchers have examined that these machine learning classifiers achieve the best performance on different datasets or under different prediction scenarios~\cite{kamei2012large, lessmann2008benchmarking, gao2016software, zimmermann2009cross}.
In RQ2, we examine whether model-agnostic based explanation tools can generate consistent explanations for the predicted buggy instances under the software defect prediction model with applied different machine learning classifiers. 

\vspace{4pt}
\noindent \textbf{RQ3:} \textit{Are the generated explanations from the same tool consistent under cross-version defect prediction scenarios?}

\vspace{4pt}

Cross-version defect prediction is one type of within-project defect prediction~\cite{turhan2009relative}, which is often used for projects that have sufficient history data, e.g., a project can have multiple releases.
One can choose different history versions as the training data to build the models with different training data selection approaches~\cite{wang2021continuous}.
%\jie{this point can be easily argued since there are studies in choosing suitable versions for model training. so here, we may say different training data selection approaches might choose diversified versions for training data. therefore, here we investigate different training versions. This is also the case for RQ4. } 
In Jiarpakdee et al.~\cite{jiarpakdee2020empirical}, the defect prediction model was trained and tested on data from the same version (i.e., within-version defect prediction).
% \song{Jiho: please double check this in the journal of Jiarpakdee's work}
% \jiho{yes, checked that they only investigate within-project and version}).  
In RQ3, we explore whether a model-agnostic based explanation tool can generate consistent explanations for the predicted buggy instances under the software defect prediction models trained on different history releases from the same project. 


\vspace{4pt}
\noindent \textbf{RQ4:} \textit{Are the generated explanations from the same tool  consistent under cross-project prediction scenarios?}

\vspace{4pt}

In cross-project defect prediction (CPDP), the training and test datasets are from different projects.
CPDP is designed for projects that do not have historical data~\cite{nam2013transfer}.
Jiarpakdee et al.~\cite{jiarpakdee2020empirical} did not examine the performance of model-agnostic based explanation in a cross-project scenario. 
In RQ4, we explore whether a model-agnostic based explanation tool can generate consistent explanations for the predicted buggy instances under the software defect prediction model trained on data from different projects. 

%\vspace{4pt}
% In RQ1, we aim to investigate the consistency of the generated explanations under different feature selection methods by getting the hit rates and ranking differences. 


%In RQ1, we aim to investigate the consistency of the generated explanations under different data sampling techniques by comparing explanations generated by the baseline and models applied with different data sampling techniques.
%In RQ2, we aim to investigate the consistency of the generated explanations under different machine learning classifiers by comparing explanations generated by the baseline and models trained with different machine learning classifiers.
%In RQ3, we aim to investigate the consistency of the generated explanations under cross-version defect prediction scenario by comparing explanations generated by data set with different version of a project.
%In RQ4, we aim to investigate the consistency of the generated explanations under cross-project defect prediction scenario by comparing explanations generated by data set with different projects.


\subsection{Experiment Data}
\label{sec:dataset}
\input{table/projs}
\input{table/features}

In this paper, to avoid potential bias introduced by experiment data, we reuse the same defect data from Jiarpakdee et al.~\cite{jiarpakdee2020empirical}, which comprises 32 releases that span 9 open-source software systems.
Table~\ref{tab:expprojects} shows the statistical information of the dataset.


For building defect prediction models, we also reuse the same software metrics used in Jiarpakdee et al.~\cite{jiarpakdee2020empirical}. In total, 65 software metrics along 3 dimensions are used, i.e., 54 code metrics (describe the relationship between properties extracted from source code and software quality), 5 process metrics (describe the relationship between development
process and software quality), and 6 human metrics (describe the relationship between the ownership of instances and software quality).
Table~\ref{tab:metrics} shows the metrics used to build defect prediction models in this work.
Note that, Jiarpakdee et  al.~\cite{jiarpakdee2020empirical} has applied AutoSpearman~\cite{jiarpakdee2018autospearman} to remove irrelevant metrics and correlated metrics before experiments.
As a result, only 22-27 of the 65 metrics were used in the experiments.
We follow the same process in this study to avoid any potential bias introduced by data pre-processing.

%The details of the metrics used as the feature is organized in Table~\ref{tab:metrics}.

\begin{comment}
\subsection{Studied Feature Selection Techniques}
\label{sec:fs}

We have used three different feature selection methods in experimenting RQ1.

\begin{itemize}
    \item \textbf{Variance Threshold method:} is a simple baseline method that removes features that have lower variance than a certain threshold.
    The threshold we used is 0.8, which removes features that has a lower variance than an 80\%.
    \item \textbf{Univariate feature selection method:} it selects features based on univariate statistical tests. Out of many different univariate statistical tests, we use one of the most common tests, the false positive rate (FPR).
    \item \textbf{L1-based feature selection method:} is a method that uses a linear model with Lasso regression to assign the importance of features. The linear model that we used for this feature selection is a simple SVM classifier.
\end{itemize}

We used the implementation of scikit-learn library \cite{scikit_learn}.
We chose these three methods because they are one of each type of feature selection method in scikit-learn which does not need to provide number of features to be selected as a hyper-parameter.
We chose these simple selectors because the focus of this study is to show how great is the impact of these simple methods have on the generated explanations.
Also, the hit rate and ranking difference are greatly affected by the number of features.
So we chose methods that results with different number of features.
\end{comment}

\subsection{Studied Data Sampling Techniques}
\label{sec:sampling}
In this study, we examine the consistency of an explanation generation tool under five widely used data sampling methods, which are shown as follows. 
\begin{itemize}
    \item \textbf{Cluster Centroids~\cite{altinccay2004clustering}}: performs an under-sampling by using centroids as the new majority samples made by k-means clusters. 
     \item \textbf{Repeated Edited Nearest Neighbours (RENN)~\cite{tomek1976experiment}}: applies the nearest-neighbour algorithm to edit the samples by removing instances that are not similar to their neighbours.
     \item \textbf{Random under-sampling (RUS)~\cite{bach2019proposal, LARADJI2015388, wahono2015systematic}}: randomly picks samples from the majority class to match the minority class.
    \item \textbf{Random over-sampling (ROS)~\cite{ling1998data, LARADJI2015388}}: over-samples the minority class by picking random samples with replacement.
    \item \textbf{SMOTE~\cite{chawla2002smote, LARADJI2015388}}: is the synthetic minority over-sampling technique (\emph{SMOTE}).
    This method creates synthetic examples of the minority class rather than over-sampling with replacements.

\end{itemize}
Researchers have widely used all the above data sampling techniques in software prediction tasks~ \cite{rodriguez2014preliminary,pak2018empirical,feng2021investigation,chen2018tackling, wang2018top,wang2013using,li2012sample}. 
In this work, we use the implementations of these data sampling techniques from the widely used imbalanced-learn Python library~\cite{imblearn}.

\subsection{Studied Defect Prediction Classifiers}
\label{sec:classifiers}
% \song{Jiho: please update the classifers and results, i.e.,  AVNNet, GBM, and xGBTree}

Jiarpakdee et al.~\cite{jiarpakdee2020empirical} showed that the model-agnostic techniques can be applied to many machine learning classifiers for explanation generation tasks.
In this study, we use the same six machine learning classifiers mentioned in Jiarpakdee et al.~\cite{jiarpakdee2020empirical} to build the defect prediction models. The details of these classifiers are as follows: 
%\nima{LR has citation but other models don't have}
\begin{itemize}
    \item \textbf{Logistic Regression}: is the baseline model used in Jiarpakdee et al.~\cite{jiarpakdee2020empirical}. 
    It is a statistical model that uses the logistic function for classifying binary dependent variables. 
    Logistic Regression is still widely used in defect prediction due to its advanced performance despite its simplicity \cite{ghotra2015revisiting}.
    \item \textbf{Decision Tree (DT):} is a model that uses trees to observe which features affect a target class.
    \item \textbf{Random Forest (RF):} utilizes ensemble learning, which is a technique that combines many classifiers to provide solutions to complex problems. A random forest algorithm consists of many decision trees and makes decisions via majority voting of multiple decision trees. 
    \item \textbf{Averaged Neural Network (AVNNet):} is a neural network model that uses models with different random numbers as seeds. It averages all the resulting models to make a prediction decision. 
    \item \textbf{Gradient Boosting Machine (GBM):} uses an additive model of a forward stage-wise fashion. It uses predictors, such as decision trees, to form an ensemble.  
    \item \textbf{Extreme Gradient Boosting Tree (xGBTree):} follows the gradient boosting principle. However, xGBTree uses a more regularized model to control over-fitting efficiently. 
    % \item \textbf{Support Vector Machine model (SVM)}: it is a statistical learning model that maps each training data points to maximize the distance between the two classes and uses those space to predict target data points.
    % \item \textbf{Naive Bayes (NB):} is one of the probabilistic classifier which bases on Bayes' theorem.
    % \item \textbf{Ensemble learning with adaptive boosting (\emph{AdaBoost}):} is a model that sums multiple weak learner's weights and results a boosted classifier. The model adapts mislabelled instances and tweaks the weak learners accordingly.
\end{itemize}
In this work, we used the implementation of the above six machine learning classifiers developed in the scikit-learn library~\cite{scikit_learn} and xgboost\footnote{\url{https://xgboost.readthedocs.io/en/latest/python/index.html}}.
Note that we have also tuned each of the six classifiers with its parameters and use the ones that can achieve the best AUC values to build prediction models in our experiments, as suggested in~\cite{jiarpakdee2020empirical}. 

\subsection{Studied Defect Prediction Scenarios}
%\jiho{Newly added this part}
Software defect prediction models can be categorized into within-project and cross-project models based on the source of the training and test datasets.
In within-project defect prediction, one can choose different history versions as the training data to build the models, which we call cross-version defect prediction. 
In this study, we investigate the consistency of explanations generated by the same tool under the two following defect prediction scenarios.

\subsubsection{Cross-Version Defect Prediction}
The Cross-version defect prediction scenario is one of the actively studied scenarios in within-project defect prediction~\cite{xu2018cross, yang2018ridge, amasaki2020cross}.
In this paper, to perform a cross-version defect prediction scenario, for each project, we use its latest version as the test version and randomly select two earlier versions as the training data to build defect prediction models respectively. 
%select one version of a data as a test data and select two versions of the same project as a training data. 
%\jiho{this is kind of different from what I did. should I change the experiment like this later?}

%Then we compare the two models to get the results.
%We evaluate all the combinations of the remaining as a training set and report the average of the results.  

\subsubsection{Cross-project Defect Prediction}

The cross-project defect prediction scenario is also another actively studied scenario in the defect prediction field~\cite{zimmermann2009cross, he2012investigation, guo2016cold}. 
To perform cross-version defect prediction, we randomly select one version from each project as the test dataset and then we randomly select two different versions from two different projects as the training data to build software defect prediction models, respectively. 

For both cross-version and cross-project defect prediction, given a test dataset, we use two different defect models to predict bugs on it, and then we run a model-agnostic based explanation generation technique to generate explanations on files that are predicted as buggy under both models to check whether the generated explanations of the same tool are consistent.  
We iterate the random selection 10 times to avoid potential bias and report the average of the results. 
%Then we compare the two models to get the results.
%We iterate the random selection for 10 times for generality and report the average of the results.
\subsection{Evaluation Measures} 
\label{sec:metric}

In this work, given a model-agnostic based explanation generation technique (i.e., \emph{LIME} and \emph{BreakDown}), we use the following two metrics to evaluate the consistency of two explanations generated by it under two different defect prediction models. They are 
%to evaluate the consistency of the explanations generated by model-agnostic based explanation generation techniques, we use two measures, i.e., 
%The two evaluation measures we use to evaluate how generated explanations are affected with different experiments are 
{\hitrate} and {\rankdiff}.

$Hit\_rate$ is the percentage of features that match between the two explanations (i.e., a set of ranked features).
For instance, Jiarpakdee et al.~\cite{jiarpakdee2020empirical} leveraged the top-10 features 
%\jiho{They used all features}
ranked by model-agnostic techniques as the explanation to interpret the prediction results.
If $N$ ($N>=0$ and $N<=10$) out of the ten features are found in two explanations generated under two different software defect prediction models, the value of {\hitrate} between these two explanations is $\frac{N}{10}$.
$Hit\_rate$ indicates how similar the two explanations are without considering the ranking orders of features in the explanations. 
%So, higher {\hitrate} means more similar are the two explanations.
The range of the {\hitrate} value is from 0.0 to 1.0.
The higher the {\hitrate}, the better the consistency of an explanation generation technique is. 
In our experiments, we use the top 10 features for \emph{LIME} and \emph{BreakDown} to calculate {\hitrate} as used in Jiarpakdee et al.~\cite{jiarpakdee2020empirical}. 
%For \emph{BreakDown}, we also the top 10 features to calculate the {\hitrate}. 
%to generate the affected features that predicts a target. 
%If six out of ten features are also found in the target model's explanation, the hit rate is 0.60.
%Note that, since \emph{LIME} uses top-k features for the explanations, \emph{BreakDown} uses all the given features, %except for the experiments that investigates different feature selection methods (RQ1), 
%\emph{BreakDown}'s {\hitrate} is always 1.0.

Note that, since {\hitrate} does not consider the order of features in the explanations, 
we also introduce {\Rankdiff}, which compares two explanations by using the orders of features in the explanations. 
Specifically, {\Rankdiff} measures the average difference of feature rankings between two explanations. 
For instance, if a feature is ranked $M$th and $H$th in two different explanations, the ranking difference of it is $ abs\left (M - H  \right )$. 
{\Rankdiff} is reported as the average ranking difference of all features in two explanations.
If a feature is not in the ranking, the difference is set to top-N. 
%{\Rankdiff} indicates how different are the generated explanation of two models by considering the ranking order of the features.
Higher {\rankdiff} means more different the explanations are by rankings.
The range of the {\rankdiff} is from zero (all features match all ranking orders) to the number of total features considered in the explanation, i.e., 10 (all features don't appear in the top 10). %and 13.48
%\song{jiho:do check this}
%\jiho{changed the value, because all features appear in breakdown, but assuming they have farthest ranks with no replacement.}
%for \emph{BreakDown} (at most all 27 features have their farthest rankings (1-27 + 2-26 + ... + 26-2 + 27-1)/27). %(1-65 + 2-64 + ... + 64-2 + 65-1) / 65). 
The smaller the {\rankdiff}, the better the consistency of an explanation generation technique is.

% \song{jiho: Approach Section updated, please check}
%{\Rankdiff} is the measure that Jiarpakdee et al.~\cite{jiarpakdee2020empirical} reported to show how consistent are the explanations when they are regenerated.

% \subsection{Baselines} 
% \label{sec:baselines}
% For each research question, we compare the baseline approach under each different method of tuning: data sampling, machine learning classifiers, and cross-version and project data set.
% The baseline model is logistic regression model with no additional tuning applied.
% This is the same baseline as Jiarpakdee et al. \cite{jiarpakdee2020empirical} used in their experiments.


==> TSE - Explainable Software Defect Prediction_ Are We There Yet_/table/RQ34.tex <==
\begin{table}[t!]
\centering
\caption{
% \song{jiho: need to be updated}
%\jiho{UPDATED}
Average {\hitrate} and {\rd} of the explanations generated by \emph{LIME} and \emph{BreakDown} under different defect prediction scenarios.}
\label{tab:rq34}
\setlength\tabcolsep{3.0pt} 
\begin{tabular}{|c|c|c|c|c|}
\hline
\multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Prediction \\ Scenario\end{tabular}}} & \multicolumn{2}{c|}{\textbf{LIME}} & \multicolumn{2}{c|}{\textbf{BreakDown}}  \\ \cline{2-5} 
  & {\hitrate} & {\rd} & {\hitrate} & {\rd} \\ \hline
\textbf{Cross-Version} & 0.518 & 6.172 & 0.591 & 5.213\\ \hline \hline
\textbf{Cross-Project} & 0.480 & 6.410 & 0.510 & 5.920\\ \hline
\end{tabular}
\end{table}

==> TSE - Explainable Software Defect Prediction_ Are We There Yet_/table/average.tex <==
%\begin{table}[]
%\centering
%\caption{Average {\hitrate} and {\rd} of \emph{LIME} and \emph{BreakDown} under different data sampling techniques. `hr' denotes {\hitrate}}
%\label{tab:average}
%\setlength\tabcolsep{3.0pt} 
%\scalebox{0.9}{
%\begin{tabular}{l|c|c|c}
%\hline
%\textbf{Sampling techniques} & \textbf{LIME\_hr} & \textbf{LIME\_rd}  & \textbf{BreakDown\_rd }\\ \hline
%Cluster Centroids & 0.600 & 5.280 &  4.963 \\ \hline
%Repeated Edited NN & 0.684 & 4.558 &  3.588 \\ \hline
%Random under-sampling & 0.619 & 5.232 &  4.058 \\ \hline
%Random over-sampling & 0.694 & 4.380 &  3.022 \\ \hline
%SMOTE & 0.685 & 4.123 &  3.086 \\ \hline 
%DT & 0.472 & 6.594 &  6.759 \\ \hline
%ENS & 0.533 & 6.202 &  6.286 \\ \hline
%NB & 0.578 & 5.796 &  6.434 \\ \hline
%RF & 0.493 & 6.333 &  6.493 \\ \hline
%SVM & 0.454 & 6.776 &  6.073 \\ \hline \hline
%CVDP & 0.601 & 5.455 &  5.519 \\ \hline \hline
%CPDP & 0.519 & 6.132 & 0.915 & 7.215 \\ \hline
%\end{tabular}
%}
%\end{table}

\begin{table}[t!]
\centering
\caption{Average {\hitrate} and {\rd} of the explanations generated by \emph{LIME} and \emph{BreakDown} under defect prediction models before and after applying different data sampling techniques.}
\label{tab:average}
\setlength\tabcolsep{3.0pt} 
\scalebox{0.95}{
\begin{tabular}{|c|c|c|c|c|}
\hline
\multicolumn{1}{|c|}{\multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Data sampling \\ techniques\end{tabular}}}} & \multicolumn{2}{c|}{\textbf{LIME}} & \multicolumn{2}{c|}{\textbf{BreakDown}} \\ \cline{2-5} 
\multicolumn{1}{|c|}{} & \hitrate & \rd & \hitrate & \rd \\ \hline
Cluster Centroids & 0.577 & 5.564 & 0.655 & 4.725 \\ \hline
Repeated Edited NN & 0.608 & 5.328 & 0.692 & 4.292 \\ \hline
Random under-sampling & 0.574 & 5.655 & 0.686 & 4.382\\ \hline
Random over-sampling & 0.641 & 4.892 & 0.769 & 3.505\\ \hline
SMOTE & 0.632 & 4.948 & 0.762 & 3.577\\ \hline \hline
\textbf{Average} &0.606&5.277&0.713&4.096\\ \hline
\end{tabular}
}
\end{table}

==> TSE - Explainable Software Defect Prediction_ Are We There Yet_/table/classifierAvg.tex <==
%\begin{table}[]
%\centering
%\caption{Average {\hitrate} and {\rd} of \emph{LIME} and \emph{BreakDown} under different data sampling techniques. `hr' denotes {\hitrate}}
%\label{tab:average}
%\setlength\tabcolsep{3.0pt} 
%\scalebox{0.9}{
%\begin{tabular}{l|c|c|c}
%\hline
%\textbf{Sampling techniques} & \textbf{LIME\_hr} & \textbf{LIME\_rd}  & \textbf{BreakDown\_rd }\\ \hline
%Cluster Centroids & 0.600 & 5.280 &  4.963 \\ \hline
%Repeated Edited NN & 0.684 & 4.558 &  3.588 \\ \hline
%Random under-sampling & 0.619 & 5.232 &  4.058 \\ \hline
%Random over-sampling & 0.694 & 4.380 &  3.022 \\ \hline
%SMOTE & 0.685 & 4.123 &  3.086 \\ \hline 
%DT & 0.472 & 6.594 &  6.759 \\ \hline
%ENS & 0.533 & 6.202 &  6.286 \\ \hline
%NB & 0.578 & 5.796 &  6.434 \\ \hline
%RF & 0.493 & 6.333 &  6.493 \\ \hline
%SVM & 0.454 & 6.776 &  6.073 \\ \hline \hline
%CVDP & 0.601 & 5.455 &  5.519 \\ \hline \hline
%CPDP & 0.519 & 6.132 & 0.915 & 7.215 \\ \hline
%\end{tabular}
%}
%\end{table}

\begin{table}[t!]
\centering
\caption{Average {\hitrate} and {\rd} of the explanations generated by \emph{LIME} and \emph{BreakDown} under  defect prediction models with different classifiers compared to the LR-based defect prediction model.
% \song{jiho: update here}
}
\label{tab:ml_avg}
\setlength\tabcolsep{3.0pt} 
\scalebox{1}{
\begin{tabular}{|l|c|c|c|c|}
\hline
\multirow{2}{*}{\textbf{Classifier}} & \multicolumn{2}{c|}{\textbf{LIME}} & \multicolumn{2}{c|}{\textbf{BreakDown}} \\ \cline{2-5} 
  & {\hitrate} & {\rd} & {\hitrate} & {\rd} \\ \hline
AVNNet & 0.613 & 5.325 & 0.681 & 4.339 \\ \hline
DT & 0.515 & 6.185 & 0.609 & 5.241 \\ \hline
GBM  & 0.559 & 5.714 & 0.638 & 4.826 \\ \hline
RF & 0.557 & 5.712 & 0.649 & 4.739 \\ \hline
XGB  & 0.570 & 5.564 & 0.641 & 4.778 \\ \hline \hline
\textbf{Average} &0.563&5.700&0.644& 4.785\\ \hline
\end{tabular}
}
\end{table}

==> TSE - Explainable Software Defect Prediction_ Are We There Yet_/table/different_ks.tex <==
% \begin{table*}[t!]
% \centering
% \caption{Average {\hitrate} and {\rd} of \emph{LIME} with different N features selected when different data sampling techniques are applied.}
% \label{tab:diff_ks}
% \resizebox{0.8\textwidth}{!}{
% \begin{tabular}{c|c|c|c|c|c|c|c|c}
% \hline
% \multirow{2}{*}{\textbf{Project}} & \multicolumn{2}{c|}{\textbf{N = 5}} & \multicolumn{2}{c|}{\textbf{N = 8}} & \multicolumn{2}{c|}{\textbf{N = 10}} & \multicolumn{2}{c}{\textbf{N = 15}} \\ \cline{2-9} 
% & {\hitrate} & {\rd} & {\hitrate} & {\rd} & {\hitrate} & {\rd} & {\hitrate} & {\rd} \\ \hline
% \textbf{Activemq} & 0.463 & 3.168 & 0.529 & 4.787 & 0.569 & 5.711 & 0.681 & 7.039 \\ \hline
% \textbf{Camel} & 0.418 & 3.451 & 0.502 & 5.027 & 0.565 & 5.493 & 0.667 & 7.253 \\ \hline
% \textbf{Derby} & 0.494 & 2.966 & 0.560 & 4.469 & 0.608 & 5.294 & 0.716 & 6.492 \\ \hline
% \textbf{Groovy} & 0.472 & 3.112 & 0.533 & 4.661 & 0.573 & 5.203 & 0.672 & 6.956 \\ \hline
% \textbf{Hbase} & 0.520 & 2.916 & 0.567 & 4.446 & 0.606 & 5.283 & 0.698 & 6.665 \\ \hline
% \textbf{Hive} & 0.486 & 3.094 & 0.556 & 4.578 & 0.583 & 5.500 & 0.679 & 6.925 \\ \hline
% \textbf{Jruby} & 0.417 & 3.430 & 0.509 & 4.915 & 0.549 & 5.862 & 0.660 & 7.247 \\ \hline
% \textbf{Lucene} & 0.494 & 3.070 & 0.576 & 4.094 & 0.595 & 5.352 & 0.676 & 6.836 \\ \hline
% \textbf{Wicket} & 0.456 & 3.161 & 0.552 & 4.616 & 0.600 & 5.465 & 0.719 & 6.551 \\ \hline \hline 
% \textbf{Overall} & 0.469 & 3.150& 0.541 & 4.62& 0.583 &5.463 & 0.685 & 6.885\\ \hline
% \end{tabular}}
% \end{table*}

% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[t!]
\centering
\caption{Average {\hitrate} and {\rd} of \emph{LIME} with different N features selected when different data sampling techniques are applied.}
\label{tab:diff_ks}
%\resizebox{0.7\textwidth}{!}{
\begin{tabular}{c|c|c|c|c|c}
\hline
\multirow{2}{*}{\textbf{Dataset}} & \textbf{N = 5} & \textbf{N = 8} & \textbf{N = 10} & \textbf{N = 15} & \textbf{N = 27/22} \\ \cline{2-6} 
 & \textbf{rank\_diff} & \textbf{rank\_diff} & \textbf{rank\_diff} & \textbf{rank\_diff} & \textbf{rank\_diff} \\ \hline
\textbf{Activemq} & 3.168 & 4.787 & 5.711 & 7.039 & 6.258 \\ \hline
\textbf{Camel} & 3.451 & 5.027 & 5.493 & 7.253 & 6.484 \\ \hline
\textbf{Derby} & 2.966 & 4.469 & 5.294 & 6.492 & 6.013 \\ \hline
\textbf{Groovy} & 3.112 & 4.661 & 5.203 & 6.956 & 6.229 \\ \hline
\textbf{Hbase} & 2.916 & 4.446 & 5.283 & 6.665 & 6.105 \\ \hline
\textbf{Hive} & 3.094 & 4.578 & 5.500 & 6.925 & 6.318 \\ \hline
\textbf{Jruby} & 3.430 & 4.915 & 5.862 & 7.247 & 6.673 \\ \hline
\textbf{Lucene} & 3.070 & 4.094 & 5.352 & 6.836 & 6.476 \\ \hline
\textbf{Wicket} & 3.161 & 4.616 & 5.465 & 6.551 & 5.414 \\ \hline
\end{tabular}%}
\end{table*}

==> TSE - Explainable Software Defect Prediction_ Are We There Yet_/table/discussion2.tex <==
\begin{table}[t!]
\centering
\vspace{-0.1in}
\caption{
% \song{jiho: need to be updated}
% \jiho{Table Updated}
Average {\hitrate} and {\rd} of \emph{LIME} and \emph{BreakDown} with different $N$ features selected.}
\label{tab:diff_ks}
\setlength\tabcolsep{6pt} 
\begin{tabular}{|c|c|c|c|c|}
\hline
\multicolumn{1}{|c|}{\multirow{2}{*}{\textbf{N}}} & \multicolumn{2}{c|}{\textbf{LIME}} & \multicolumn{2}{c|}{\textbf{BreakDown}}  \\ \cline{2-5} 
\multicolumn{1}{|l|}{} & {\hitrate} & {\rd} & {\hitrate} & {\rd}\\ \hline
\textbf{5} & 0.522 & 2.914 & 0.650 & 2.279 \\ \hline
\textbf{8} & 0.571 & 4.416 & 0.686 & 3.446 \\ \hline
\textbf{10} & 0.606 & 5.277 & 0.713 & 4.096 \\ \hline
\textbf{15} & 0.713 & 6.788 & 0.776 & 5.229 \\ \hline
%\textbf{all} & 1.000 & 5.099 & 1.000 & 3.701 \\ \hline
\end{tabular}
\end{table}

==> TSE - Explainable Software Defect Prediction_ Are We There Yet_/table/features.tex <==
\begin{table*}[t]
	\centering
	\caption{Details of the metrics used to build software bug prediction models in this work.}
	\label{tab:metrics}
	\scalebox{0.9}{
\setlength\tabcolsep{4pt} 
\begin{tabular}{l|l|l}
\hline
\textbf{Type} & \textbf{Metrics} & \textbf{Count} \\ \hline
File   &  \begin{tabular}[c]{@{}l@{}}AvgCyclomatic, AvgCyclomaticModified, AvgCyclomaticStrict, AvgEssential, AvgLine, AvgLineBlank, AvgLineCode, AvgLineComment, \\ CountDeclClass, CountDeclClassMethod, CountDeclClassVariable, CountDeclFunction, CountDeclInstanceMethod,\\ CountDeclInstanceVariable, CountDeclMethod, CountDeclMethodDefault, CountDeclMethodPrivate, CountDeclMethodProtected,\\ CountDeclMethodPublic, CountLine, CountLineBlank, CountLineCode, CountLineCodeDecl, CountLineCodeExe, CountLineComment,\\ CountSemicolon, CountStmt, CountStmtDecl, CountStmtExe, MaxCyclomatic, MaxCyclomaticModified, MaxCyclomaticStrict, \\ RatioCommentToCode, SumCyclomatic, SumCyclomaticModified, SumCyclomaticStrict, SumEssential\end{tabular} & 37 \\ \hline
Class  & CountClassBase, CountClassCoupled, CountClassDerived, MaxInheritanceTree, PercentLackOfCohesion& 5 \\ \hline
Method & CountInput\_\{Min, Mean, Max\}, CountOutput\_\{Min, Mean, Max\}, CountPath\_\{Min, Mean, Max\}, MaxNesting\_\{Min, Mean, Max\}& 12 \\ \hline
Process & COMM, ADDED\_LINES, DEL\_LINES, ADEV, DDEV & 5 \\ \hline
Ownership & MINOR\_COMMIT, MINOR\_LINE, MAJOR\_COMMIT, MAJOR\_LINE, OWN\_COMMIT, OWN\_LINE & 6 \\ \hline
\end{tabular}
}
%\vspace{-0.12in}
\end{table*}

==> TSE - Explainable Software Defect Prediction_ Are We There Yet_/table/projs.tex <==
\begin{table}[t!]
\centering
\caption{Subjects studied in this work} 
%\textbf{``\% of versions''} is the percentage of selected versions from a project.}
\label{tab:expprojects}
\scalebox{0.95}{
\setlength\tabcolsep{3pt} 
\begin{tabular}{l|c|c|c|l}
\hline
\textbf{Project}  &\textbf{\#Files} & \textbf{\#KLOC} & \textbf{Bug rate} & \textbf{Studied Releases}  \\ \hline
ActiveMQ &  1.8K-3.4K  & 142-299 &  6\%-15\% & 5.0,5.1,5.2,5.3,5.8  \\ \hline
Camel &   1.5K-8.8K &  75-383 &2\%-18\% &1.4,2.9,2.10,2.11  \\ \hline
Derby & 1.9K-2.7K &  412-533 &14\%-33\% &10.2,10.3,10.5  \\ \hline
Groovy & 0.7K-0.9K&74-90 & 3\%-8\% & 1.5.7,1.6.0.b1,1.6.0.b2  \\ \hline
HBase & 10K-18K &  246-534  &  20\%-26\% & 0.94,0.95.0,0.95.2 \\ \hline
Hive &   14K-27K  & 287-563  &  8\%-19\% & 0.9,0.10,0.12 \\ \hline
JRuby &   0.7K-16K  & 105-238 & 5\%-18\% & 1.1,1.4,1.5,1.7 \\ \hline
Lucene &  0.8K-28K  &   101-342 &  3\%-24\% & 2.3,2.9,3.0,3.1 \\ \hline
Wicket &  16K-28K  &109-165  & 4\%-7\% & 1.3.b1,1.3.b2,1.5.3 \\ \hline
\end{tabular}
}
\end{table}

==> TSE - Explainable Software Defect Prediction_ Are We There Yet_/table/rq1.tex <==
\begin{table*}[!ht]
\centering
\caption{Result of RQ1, comparison of models with different data sampling techniques applied.} 
%\textbf{``\% of versions''} is the percentage of selected versions from a project.}
\label{tab:rq1}
\begin{subtable}[hbt!]{1\textwidth}
\centering
\resizebox{0.85\textwidth}{!}{
\begin{tabular}{l|l|l|l|l|l|l|l|l|l|l}
\hline
\textbf{LIME (top\_k: 10)} & \multicolumn{2}{l|}{\textbf{Random Under}} & \multicolumn{2}{l|}{\textbf{Repeated Edited NN}} & \multicolumn{2}{l|}{\textbf{Cluster Centroids}} & \multicolumn{2}{l|}{\textbf{SMOTE}} & \multicolumn{2}{l}{\textbf{Random Over}} \\ \hline
Data set & {\hitrate} & {\rd} & {\hitrate} & {\rd} & {\hitrate} & {\rd} & {\hitrate} & {\rd} & {\hitrate} & {\rd} \\ \hline
activemq-5.0.0 & 0.499 & 6.167 & 0.510 & 6.191 & 0.520 & 6.196 & 0.610 & 4.938 & 0.587 & 5.100 \\ \hline
activemq-5.1.0 & 0.530 & 6.269 & 0.623 & 5.278 & 0.573 & 5.634 & 0.641 & 5.238 & 0.642 & 5.108 \\ \hline
activemq-5.2.0 & 0.480 & 6.548 & 0.545 & 5.970 & 0.518 & 6.091 & 0.534 & 6.044 & 0.422 & 6.847 \\ \hline
activemq-5.3.0 & 0.540 & 6.280 & 0.555 & 6.096 & 0.560 & 5.807 & 0.654 & 4.918 & 0.672 & 4.921 \\ \hline
activemq-5.8.0 & 0.597 & 5.574 & 0.618 & 5.688 & 0.528 & 5.880 & 0.590 & 5.117 & 0.661 & 4.294 \\ \hline
camel-1.4.0 & 0.610 & 5.086 & 0.579 & 5.279 & 0.574 & 5.285 & 0.715 & 3.909 & 0.696 & 4.311 \\ \hline
camel-2.9.0 & 0.620 & 5.222 & 0.603 & 5.643 & 0.481 & 6.303 & 0.779 & 3.971 & 0.728 & 4.274 \\ \hline
camel-2.10.0 & 0.582 & 5.660 & 0.734 & 4.097 & 0.498 & 6.583 & 0.775 & 3.750 & 0.764 & 3.577 \\ \hline
camel-2.11.0 & 0.549 & 5.917 & 0.529 & 6.176 & 0.401 & 7.336 & 0.766 & 4.485 & 0.765 & 4.491 \\ \hline
derby-10.2.1.6 & 0.372 & 6.759 & 0.332 & 7.233 & 0.378 & 6.601 & 0.367 & 6.752 & 0.383 & 6.558 \\ \hline
derby-10.3.1.4 & 0.365 & 6.854 & 0.327 & 7.384 & 0.359 & 6.824 & 0.360 & 6.887 & 0.356 & 6.909 \\ \hline
derby-10.5.1.1 & 0.350 & 7.039 & 0.332 & 7.098 & 0.359 & 6.824 & 0.330 & 7.249 & 0.322 & 7.269 \\ \hline
groovy-1\_5\_7 & 0.473 & 6.644 & 0.498 & 6.505 & 0.307 & 7.281 & 0.657 & 5.402 & 0.640 & 5.641 \\ \hline
groovy-1\_6\_BETA\_1 & 0.523 & 6.146 & 0.545 & 5.673 & 0.605 & 5.418 & 0.601 & 5.300 & 0.657 & 4.744 \\ \hline
groovy-1\_6\_BETA\_2 & 0.635 & 4.783 & 0.564 & 5.331 & 0.469 & 6.263 & 0.684 & 4.504 & 0.689 & 4.272 \\ \hline
hbase-0.94.0 & 0.553 & 5.739 & 0.510 & 5.953 & 0.569 & 5.491 & 0.589 & 5.281 & 0.603 & 4.989 \\ \hline
hbase-0.95.0 & 0.679 & 4.258 & 0.665 & 4.745 & 0.670 & 4.632 & 0.700 & 4.015 & 0.723 & 3.888 \\ \hline
hbase-0.95.2 & 0.603 & 5.065 & 0.595 & 4.974 & 0.625 & 4.718 & 0.614 & 4.706 & 0.619 & 4.816 \\ \hline
hive-0.9.0 & 0.736 & 4.492 & 0.721 & 5.098 & 0.765 & 4.070 & 0.802 & 3.361 & 0.748 & 4.221 \\ \hline
hive-0.10.0 & 0.592 & 5.408 & 0.594 & 5.254 & 0.557 & 5.401 & 0.609 & 5.022 & 0.576 & 5.208 \\ \hline
hive-0.12.0 & 0.474 & 6.632 & 0.632 & 5.244 & 0.693 & 4.614 & 0.249 & 8.286 & 0.418 & 6.399 \\ \hline
jruby-1.1 & 0.613 & 5.074 & 0.625 & 4.674 & 0.615 & 4.782 & 0.667 & 4.539 & 0.675 & 4.453 \\ \hline
jruby-1.4.0 & 0.644 & 4.723 & 0.709 & 4.021 & 0.661 & 4.683 & 0.645 & 4.712 & 0.674 & 4.552 \\ \hline
jruby-1.5.0 & 0.322 & 7.265 & 0.347 & 7.171 & 0.338 & 7.065 & 0.369 & 6.845 & 0.295 & 7.681 \\ \hline
jruby-1.7.0.preview1 & 0.624 & 4.960 & 0.767 & 3.538 & 0.535 & 5.567 & 0.613 & 4.905 & 0.594 & 5.154 \\ \hline
lucene-2.3.0 & 0.431 & 6.489 & 0.407 & 6.854 & 0.418 & 6.407 & 0.388 & 6.961 & 0.422 & 6.519 \\ \hline
lucene-2.9.0 & 0.406 & 6.496 & 0.445 & 6.114 & 0.390 & 6.755 & 0.424 & 6.453 & 0.403 & 6.625 \\ \hline
lucene-3.0.0 & 0.552 & 5.978 & 0.549 & 5.435 & 0.521 & 5.629 & 0.540 & 5.755 & 0.491 & 6.208 \\ \hline
lucene-3.1 & 0.421 & 6.370 & 0.452 & 6.279 & 0.380 & 6.744 & 0.377 & 6.786 & 0.356 & 6.971 \\ \hline
wicket-1.3.0-beta2 & 0.436 & 6.552 & 0.564 & 5.577 & 0.636 & 4.717 & 0.519 & 6.218 & 0.691 & 4.286 \\ \hline
wicket-1.3.0-incubating-beta-1 & 0.575 & 6.020 & 0.567 & 5.900 & 0.690 & 4.729 & 0.614 & 5.133 & 0.668 & 4.761 \\ \hline
wicket-1.5.3 & 0.436 & 6.552 & 0.564 & 5.577 & 0.518 & 5.658 & 0.519 & 6.218 & 0.594 & 5.126 \\ \hline \hline
average & 0.526	& 5.907	& 0.550	& 5.689	& 0.522	& 5.812	& 0.572	& 5.427	& 0.579	& 5.318 \\ \hline
\end{tabular}}
\caption{Result of Lime}
\label{tab:rq1_lime}

\centering
\resizebox{0.7\textwidth}{!}{
\begin{tabular}{l|l|l|l|l|l}
\hline
\textbf{BreakDown} & \textbf{Random Under} & \textbf{RepeatedEditedNN} & \textbf{Cluster Centroid} & \textbf{SMOTE} & \textbf{Random Over} \\ \hline
Data set & {\rd} & {\rd} & {\rd} & {\rd} & {\rd} \\ \hline
activemq-5.0.0 & 12.846 & 12.011 & 13.213 & 9.273 & 10.141 \\ \hline
activemq-5.1.0 & 14.035 & 10.158 & 13.047 & 9.631 & 9.444 \\ \hline
activemq-5.2.0 & 13.725 & 9.190 & 12.130 & 9.794 & 12.177 \\ \hline
activemq-5.3.0 & 13.776 & 12.315 & 11.387 & 6.864 & 6.226 \\ \hline
activemq-5.8.0 & 15.516 & 12.298 & 17.510 & 15.458 & 12.872 \\ \hline
camel-1.4.0 & 10.263 & 14.841 & 11.010 & 6.531 & 6.068 \\ \hline
camel-2.9.0 & 15.799 & 14.932 & 17.798 & 10.163 & 12.053 \\ \hline
camel-2.10.0 & 14.953 & 7.995 & 17.477 & 8.740 & 7.852 \\ \hline
camel-2.11.0 & 14.435 & 11.794 & 17.850 & 8.318 & 8.014 \\ \hline
derby-10.2.1.6 & 11.057 & 16.629 & 9.912 & 10.573 & 10.538 \\ \hline
derby-10.3.1.4 & 13.407 & 14.787 & 11.980 & 13.103 & 13.179 \\ \hline
derby-10.5.1.1 & 30.768 & 23.622 & 11.980 & 30.260 & 29.913 \\ \hline
groovy-1\_5\_7 & 17.824 & 14.109 & 25.660 & 12.610 & 11.769 \\ \hline
groovy-1\_6\_BETA\_1 & 14.993 & 13.419 & 17.466 & 11.396 & 11.400 \\ \hline
groovy-1\_6\_BETA\_2 & 13.113 & 15.767 & 13.828 & 8.391 & 9.805 \\ \hline
hbase-0.94.0 & 11.230 & 15.892 & 10.205 & 10.389 & 8.654 \\ \hline
hbase-0.95.0 & 9.526 & 13.912 & 11.389 & 7.619 & 8.248 \\ \hline
hbase-0.95.2 & 9.499 & 11.833 & 7.605 & 8.008 & 7.993 \\ \hline
hive-0.9.0 & 9.525 & 14.868 & 9.171 & 5.506 & 5.529 \\ \hline
hive-0.10.0 & 12.679 & 16.721 & 17.274 & 21.125 & 20.744 \\ \hline
hive-0.12.0 & 16.634 & 15.524 & 15.015 & 22.747 & 22.847 \\ \hline
jruby-1.1 & 13.616 & 13.867 & 12.661 & 6.838 & 8.024 \\ \hline
jruby-1.4.0 & 11.471 & 15.420 & 12.257 & 8.342 & 7.914 \\ \hline
jruby-1.5.0 & 19.345 & 21.558 & 22.428 & 28.776 & 28.820 \\ \hline
jruby-1.7.0.preview1 & 13.597 & 6.123 & 19.962 & 10.212 & 13.167 \\ \hline
lucene-2.3.0 & 23.679 & 17.670 & 11.901 & 22.809 & 24.242 \\ \hline
lucene-2.9.0 & 19.768 & 16.680 & 17.425 & 25.349 & 25.444 \\ \hline
lucene-3.0.0 & 15.252 & 8.356 & 18.586 & 17.474 & 15.487 \\ \hline
lucene-3.1 & 25.741 & 15.609 & 14.209 & 27.745 & 27.684 \\ \hline
wicket-1.3.0-beta2 & 14.989 & 8.164 & 14.627 & 12.434 & 10.431 \\ \hline
wicket-1.3.0-incubating-beta-1 & 12.371 & 9.098 & 13.031 & 14.005 & 7.723 \\ \hline
wicket-1.5.3 & 14.614 & 8.164 & 14.627 & 12.194 & 9.317 \\ \hline \hline
average & 15.001 & 13.541 & 14.520 & 13.521 & 13.241 \\ \hline
\end{tabular}}
\caption{Result of BreakDown}
\label{tab:rq1_bd}

\end{subtable}
\end{table*}



==> TSE - Explainable Software Defect Prediction_ Are We There Yet_/table/rq2.tex <==
\begin{table*}[!ht]
\centering
\caption{Result of RQ2, comparison of different machine learning algorithms } 
%\textbf{``\% of versions''} is the percentage of selected versions from a project.}
\label{tab:rq2}
\begin{subtable}[hbt!]{1\textwidth}
\centering
\resizebox{0.8\textwidth}{!}{
\begin{tabular}{l|l|l|l|l|l|l|l|l|l|l}
\hline
LIME  & \multicolumn{2}{l|}{SVM} & \multicolumn{2}{l|}{NB (Gaussian)} & \multicolumn{2}{l|}{RF} & \multicolumn{2}{l|}{Ensemble(Adaboost)} & \multicolumn{2}{l}{DT} \\ \hline
Data sets & {\hitrate}  & {\rd} & {\hitrate} & {\rd} & {\hitrate}  & {\rd} & {\hitrate}  & {\rd} & {\hitrate}  & {\rd} \\ \hline
activemq-5.0.0 & 0.360 & 7.380 & 0.308 & 8.077  & 0.292  & 7.930  & 0.258  & 8.213  & 0.249  & 8.441  \\ \hline
activemq-5.1.0 & N/A & N/A & 0.277 & 7.957  & 0.331  & 7.759  & 0.225  & 8.101  & 0.242  & 8.360  \\ \hline
activemq-5.2.0 & N/A & N/A & 0.461 & 6.520  & 0.104  & 9.284  & 0.202  & 8.476  & 0.119  & 9.242  \\ \hline
activemq-5.3.0 & 0.267 & 8.233 & 0.218 & 8.711  & 0.257  & 8.093  & 0.157  & 9.012  & 0.190  & 8.794  \\ \hline
activemq-5.8.0 & N/A & N/A & 0.297 & 7.588  & 0.219  & 8.471  & 0.247  & 8.236  & 0.172  & 8.725  \\ \hline
camel-1.4.0  & 0.467 & 7.117 & 0.389 & 7.037  & 0.239  & 8.330  & 0.201  & 8.682  & 0.258  & 8.220  \\ \hline
camel-2.9.0  & N/A & N/A & 0.597 & 5.361  & 0.475  & 6.688  & 0.270  & 8.100  & 0.250  & 8.404  \\ \hline
camel-2.10.0 & N/A & N/A & 0.306 & 8.035  & 0.325  & 7.688  & 0.156  & 8.756  & 0.250  & 8.248  \\ \hline
camel-2.11.0 & N/A & N/A & 0.444 & 6.982  & 0.200  & 8.900  & 0.200  & 9.100  & 0.325  & 7.738  \\ \hline
derby-10.2.1.6 & 0.357 & 6.821 & 0.384 & 6.610  & 0.185  & 8.692  & 0.215  & 8.496  & 0.204  & 8.551  \\ \hline
derby-10.3.1.4 & 0.329 & 7.057 & 0.377 & 6.712  & 0.148  & 9.006  & 0.245  & 8.368  & 0.209  & 8.551  \\ \hline
derby-10.5.1.1 & 0.320 & 7.400 & 0.420 & 6.653  & 0.134  & 9.174  & 0.171  & 8.855  & 0.171  & 8.971  \\ \hline
groovy-1\_5\_7 & N/A & N/A & 0.347 & 7.520  & 0.270  & 8.300  & 0.287  & 7.963  & 0.081  & 9.506  \\ \hline
groovy-1\_6\_BETA\_1 & N/A & N/A & 0.408 & 6.806  & 0.331  & 7.770  & 0.222  & 8.296  & 0.233  & 8.317  \\ \hline
groovy-1\_6\_BETA\_2 & 0.200 & 8.100 & 0.399 & 6.667  & 0.170  & 9.095  & 0.170  & 8.880  & 0.185  & 8.848  \\ \hline
hbase-0.94.0 & 0.300 & 8.300 & 0.591 & 5.628  & 0.223  & 8.442  & 0.129  & 9.141  & 0.178  & 8.749  \\ \hline
hbase-0.95.0 & 0.200 & 8.300 & 0.233 & 7.933  & 0.108  & 9.183  & 0.237  & 8.328  & 0.140  & 9.116  \\ \hline
hbase-0.95.2 & 0.200 & 8.500 & 0.253 & 7.767  & 0.187  & 8.558  & 0.321  & 7.784  & 0.156  & 9.045  \\ \hline
hive-0.9.0 & 0.204 & 8.796 & 0.753 & 4.734  & 0.488  & 6.384  & 0.266  & 8.218  & 0.232  & 8.447  \\ \hline
hive-0.10.0  & 0.200 & 8.375 & 0.520 & 5.580  & 0.350  & 7.917  & 0.233  & 8.743  & 0.347  & 7.839  \\ \hline
hive-0.12.0  & N/A & N/A & 0.650 & 4.912  & 0.300  & 7.700  & 0.400  & 7.900  & 0.300  & 8.050  \\ \hline
jruby-1.1 & 0.200 & 8.100 & 0.260 & 7.600  & 0.223  & 8.716  & 0.285  & 8.095  & 0.145  & 9.058  \\ \hline
jruby-1.4.0  & 0.233 & 8.200 & 0.275 & 7.429  & 0.289  & 8.004  & 0.192  & 8.434  & 0.194  & 8.713  \\ \hline
jruby-1.5.0  & 0.325 & 7.600 & 0.375 & 6.738  & 0.140  & 9.290  & 0.225  & 8.790  & 0.194  & 8.678  \\ \hline
jruby-1.7.0.preview1 & N/A & N/A & 0.464 & 6.171  & 0.290  & 7.920  & 0.378  & 7.433  & 0.273  & 8.225  \\ \hline
lucene-2.3.0 & N/A & N/A & 0.460 & 5.973  & 0.173  & 8.863  & 0.223  & 8.586  & 0.233  & 8.445  \\ \hline
lucene-2.9.0 & 0.400 & 7.100 & 0.275 & 7.500  & 0.208  & 8.658  & 0.231  & 8.450  & 0.210  & 8.670  \\ \hline
lucene-3.0.0 & N/A & N/A & 0.267 & 7.633  & 0.233  & 8.533  & 0.267  & 8.411  & 0.267  & 8.100  \\ \hline
lucene-3.1 & N/A & N/A & 0.467 & 6.167  & 0.100  & 9.200  & 0.233  & 8.400  & 0.204  & 8.598  \\ \hline
wicket-1.3.0-beta2 & N/A & N/A & 0.419 & 6.527  & 0.333  & 7.849  & 0.261  & 8.310  & 0.245  & 8.340  \\ \hline
wicket-1.3.0-incubating-beta-1 & N/A & N/A & 0.418 & 6.590  & 0.175  & 8.881  & 0.252  & 8.256  & 0.168  & 9.024  \\ \hline
wicket-1.5.3 & N/A & N/A & 0.518 & 6.021  & 0.280  & 7.880  & 0.231  & 8.474  & 0.197  & 8.739  \\ \hline \hline
average & 0.285 & 7.836 & 0.401 & 6.817 & 0.243 & 8.349 & 0.237 & 8.415 & 0.213 & 8.586 \\ \hline
\end{tabular}}
\caption{Result of Lime}
\label{tab:rq2_lime}

\centering
\resizebox{0.55\textwidth}{!}{
\begin{tabular}{l|l|l|l|l|l}
\hline
BreakDown & SVM & NB & RF & Ensemble & DT \\ \hline
Data set  & {\rd} & {\rd} & {\rd} & {\rd} & {\rd} \\ \hline
activemq-5.0.0 & 15.506 & 19.632 & 20.572 & 18.892 & 20.415 \\ \hline
activemq-5.1.0 & N/A & 19.516 & 19.184 & 21.686 & 21.376 \\ \hline
activemq-5.2.0 & N/A & 20.293 & 18.999 & 17.582 & 19.286 \\ \hline
activemq-5.3.0 & 15.015 & 19.128 & 19.212 & 20.049 & 19.606 \\ \hline
activemq-5.8.0 & N/A & 22.520 & 22.677 & 20.527 & 21.596 \\ \hline
camel-1.4.0  & 17.236 & 19.176 & 18.877 & 19.857 & 20.251 \\ \hline
camel-2.9.0  & N/A & 18.846 & 20.137 & 18.283 & 21.006 \\ \hline
camel-2.10.0 & N/A & 16.821 & 19.158 & 20.282 & 20.056 \\ \hline
camel-2.11.0 & N/A & 16.633 & 17.754 & 19.600 & 17.635 \\ \hline
derby-10.2.1.6 & 12.454 & 11.409 & 17.675 & 20.671 & 19.512 \\ \hline
derby-10.3.1.4 & 16.114 & 14.860 & 18.814 & 21.447 & 21.141 \\ \hline
derby-10.5.1.1 & 30.468 & 31.042 & 30.030 & 22.971 & 26.149 \\ \hline
groovy-1\_5\_7 & N/A & 20.697 & 21.418 & 20.486 & 22.056 \\ \hline
groovy-1\_6\_BETA\_1 & N/A & 23.099 & 21.947 & 19.394 & 21.050 \\ \hline
groovy-1\_6\_BETA\_2 & 11.692 & 22.562 & 20.163 & 19.872 & 20.403 \\ \hline
hbase-0.94.0 & 15.323 & 21.630 & 22.351 & 19.369 & 20.312 \\ \hline
hbase-0.95.0 & 18.538 & 20.487 & 21.834 & 19.576 & 21.818 \\ \hline
hbase-0.95.2 & 18.092 & 21.187 & 21.377 & 19.421 & 20.378 \\ \hline
hive-0.9.0 & 18.694 & 19.031 & 19.982 & 21.200 & 20.033 \\ \hline
hive-0.10.0  & 15.808 & 22.138 & 20.558 & 19.649 & 21.521 \\ \hline
hive-0.12.0  & N/A & 24.107 & 23.785 & 22.954 & 19.477 \\ \hline
jruby-1.1 & 22.892 & 20.945 & 20.774 & 19.320 & 21.124 \\ \hline
jruby-1.4.0  & 21.041 & 21.067 & 21.908 & 19.448 & 22.109 \\ \hline
jruby-1.5.0  & 29.046 & 27.131 & 29.692 & 22.329 & 23.019 \\ \hline
jruby-1.7.0.preview1 & N/A & 20.765 & 23.582 & 19.275 & 21.260 \\ \hline
lucene-2.3.0 & N/A & 26.658 & 23.277 & 20.349 & 22.034 \\ \hline
lucene-2.9.0 & 25.908 & 26.292 & 27.333 & 22.568 & 24.386 \\ \hline
lucene-3.0.0 & N/A & 21.938 & 20.400 & 20.701 & 21.067 \\ \hline
lucene-3.1 & N/A & 27.908 & 22.246 & 19.713 & 20.822 \\ \hline
wicket-1.3.0-beta2 & N/A & 20.245 & 20.607 & 20.133 & 20.963 \\ \hline
wicket-1.3.0-incubating-beta-1 & N/A & 18.926 & 19.612 & 18.186 & 20.249 \\ \hline
wicket-1.5.3 & N/A & 18.280 & 17.600 & 17.886 & 18.911 \\ \hline \hline
average & 18.989 & 21.093 & 21.360 & 20.115 & 20.969 \\ \hline
\end{tabular}}
\caption{Result of BreakDown}
\label{tab:rq2_bd}

\end{subtable}
\end{table*}



==> figure/rq1/rq1_combine.tex <==
\begin{figure*}[th!]
\centering
\begin{subfigure}{0.24\linewidth}
\centering
\input{figure/rq1/vt_lime_hr}
\vspace{-0.2in}
\caption{\emph{LIME} {\hitrate}}
%\vspace{-0.1in}
\end{subfigure}\hfill
\begin{subfigure}{0.24\linewidth}
\centering
\input{figure/rq1/vt_bd_hr}
\vspace{-0.2in}
\caption{\emph{BreakDown} {\hitrate}}
%\vspace{-0.1in}
\end{subfigure}\hfill
\begin{subfigure}{0.24\linewidth}
\centering
\input{figure/rq1/vt_lime_rd}
\vspace{-0.2in}
\caption{\emph{LIME} {\rd}}
%\vspace{-0.1in}
\end{subfigure}\hfill
\begin{subfigure}{0.24\linewidth}
\centering
\input{figure/rq1/vt_bd_rd}
\vspace{-0.2in}
\caption{\emph{BreakDown} {\rd}}
%\vspace{-0.1in}
\end{subfigure}\hfill

\centering
\begin{subfigure}{0.24\linewidth}
\centering
\input{figure/rq1/svc_lime_hr}
\vspace{-0.2in}
\caption{\emph{LIME} {\hitrate}}
%\vspace{-0.1in}
\end{subfigure}\hfill
\begin{subfigure}{0.24\linewidth}
\centering
\input{figure/rq1/svc_bd_hr}
\vspace{-0.2in}
\caption{\emph{BreakDown} {\hitrate}}
%\vspace{-0.1in}
\end{subfigure}\hfill
\begin{subfigure}{0.24\linewidth}
\centering
\input{figure/rq1/svc_lime_rd}
\vspace{-0.2in}
\caption{\emph{LIME} {\rd}}
%\vspace{-0.1in}
\end{subfigure}\hfill
\begin{subfigure}{0.24\linewidth}
\centering
\input{figure/rq1/svc_bd_rd}
\vspace{-0.2in}
\caption{\emph{BreakDown} {\rd}}
%\vspace{-0.1in}
\end{subfigure}\hfill

\centering
\begin{subfigure}{0.24\linewidth}
\centering
\input{figure/rq1/fpr_lime_hr}
\vspace{-0.2in}
\caption{\emph{LIME} {\hitrate}}
%\vspace{-0.1in}
\end{subfigure}\hfill
\begin{subfigure}{0.24\linewidth}
\centering
\input{figure/rq1/fpr_bd_hr}
\vspace{-0.2in}
\caption{\emph{BreakDown} {\hitrate}}
%\vspace{-0.1in}
\end{subfigure}\hfill
\begin{subfigure}{0.24\linewidth}
\centering
\input{figure/rq1/fpr_lime_rd}
\vspace{-0.2in}
\caption{\emph{LIME} {\rd}}
%\vspace{-0.1in}
\end{subfigure}\hfill
\begin{subfigure}{0.24\linewidth}
\centering
\input{figure/rq1/fpr_bd_rd}
\vspace{-0.2in}
\caption{\emph{BreakDown} {\rd}}
%\vspace{-0.1in}
\end{subfigure}\hfill

\vspace{-0.1in}
\caption{ \small
This is the {\hitrate} and {\rd} comparison of different feature selection method applied.
(a) $\sim$ (d) is the result of Variance Threshold Feature Selection Method.
(e) $\sim$ (h) is the result of SelectFromModel (L1 norm) Feature Selection Method.
(i) $\sim$ (l) is the result of Univariate Feature Selection Method (FPR).
}
\label{fig:rq1_comb}
\vspace{-0.1in}
\end{figure*}
%\vspace{-0.1in}


==> figure/rq3.tex <==
\begin{figure}
\captionsetup[subfigure]{justification=centering}
    % hit rate part of figure
    \begin{subfigure}[]{\linewidth}
        \begin{tikzpicture}
        \begin{axis}[
        ymax=2,
        ymin=0,
        y=1.5cm,
        xtick={0.0,0.2,0.4,0.6,0.8,1.0},
        xticklabels={0.0,0.2,0.4,0.6,0.8,1.0},
        ytick={1},
        yticklabels={\qquad \, LIME},
        axis y line=left,
        axis x line=bottom,
        xmin=0.0,
        xmax=1.0,
        %ytick={1,2,3},
        %yticklabels={Group A, Group B, Group C},
        ]
        \addplot+[black,thick,
        boxplot prepared={
            draw position=1,
            lower whisker=0.320,
            lower quartile=0.488,
            median=0.541,
            upper quartile=0.629,
            upper whisker=0.791,
        },/pgf/number format/precision=0
        ]
        coordinates {}
        [above]
        node at
        (boxplot box cs: \boxplotvalue{lower whisker},1){}
        node at
        (boxplot box cs: \boxplotvalue{lower quartile},1){}
        node at
        (boxplot box cs: \boxplotvalue{median},1){}
        node at
        (boxplot box cs: \boxplotvalue{upper quartile},1){}
        node at
        (boxplot box cs: \boxplotvalue{upper whisker},1){}
        ;
        
        \end{axis}
        \end{tikzpicture}
        \caption{{\hitrate} of \emph{LIME}}
        \label{fig:rq3_hitrate}
        
    \end{subfigure}

    % rank_diff part of figure
    \begin{subfigure}[]{\linewidth}
        \begin{tikzpicture}
        \begin{axis}[
        ymax=3.5,
        ymin=0,
        y=1.5cm,
        xtick={3,6,...,23},
        xticklabels={3,6,...,23},
        ytick={1,2.5},
        yticklabels={BreakDown, LIME},
        axis y line=left,
        axis x line=bottom,
        xmin=3,
        xmax=23,
        %ytick={1,2,3},
        %yticklabels={Group A, Group B, Group C},
        ]
        \addplot+[black,thick,
        boxplot prepared={
            draw position=2.5,
            lower whisker=3.357,
            lower quartile=4.765,
            median=5.834,
            upper quartile=6.322,
            upper whisker=7.291,
        },/pgf/number format/precision=0
        ]
        coordinates {}
        [above]
        node at
        (boxplot box cs: \boxplotvalue{lower whisker},1){}
        node at
        (boxplot box cs: \boxplotvalue{lower quartile},1){}
        node at
        (boxplot box cs: \boxplotvalue{median},1){}
        node at
        (boxplot box cs: \boxplotvalue{upper quartile},1){}
        node at
        (boxplot box cs: \boxplotvalue{upper whisker},1){}
        ;
         \addplot+[black,thick,
        boxplot prepared={
            draw position=1,
            lower whisker=3.940,
            lower quartile=10.106,
            median=12.444,
            upper quartile=14.698,
            upper whisker=18.923,
        },/pgf/number format/precision=0
        ]
        coordinates {(1,22.913) (1,24.919)}
        [above]
        node at
        (boxplot box cs: \boxplotvalue{lower whisker},1){}
        node at
        (boxplot box cs: \boxplotvalue{lower quartile},1){}
        node at
        (boxplot box cs: \boxplotvalue{median},1){}
        node at
        (boxplot box cs: \boxplotvalue{upper quartile},1){}
        node at
        (boxplot box cs: \boxplotvalue{upper whisker},1){}
        ;
        \end{axis}
        \end{tikzpicture}
        \caption{{\rankdiff} of \emph{LIME} and \emph{BreakDown}}
        \label{fig:rq3_rankdiff}
    \end{subfigure}
    \caption{Result of RQ3, comparing explanations in cross-version defect prediction scenario}
    \label{fig:rq3}
\end{figure}


==> figure/rq3/rq3_combine.tex <==
\begin{figure*}[th!]

\centering 
\begin{subfigure}{0.20\linewidth}
\centering
\includegraphics[width=\textwidth]{figure/rq3/rq3_dt_lime_hr.png}
\vspace{-0.2in}
\caption{Decision Tree}
%\vspace{-0.1in}
\end{subfigure}\hfill
\begin{subfigure}{0.20\linewidth}
\centering
\includegraphics[width=\textwidth]{figure/rq3/rq3_ens_lime_hr.png}
\vspace{-0.2in}
\caption{Ensemble}
%\vspace{-0.1in}
\end{subfigure}\hfill
\begin{subfigure}{0.20\linewidth}
\centering
\includegraphics[width=\textwidth]{figure/rq3/rq3_gnb_lime_hr.png}
\vspace{-0.2in}
\caption{NaiveBayes}
%\vspace{-0.1in}
\end{subfigure}\hfill
\centering
\begin{subfigure}{0.20\linewidth}
\centering
\includegraphics[width=\textwidth]{figure/rq3/rq3_rf_lime_hr.png}
\vspace{-0.2in}
\caption{RandomForest}
%\vspace{-0.1in}
\end{subfigure}\hfill
\centering
\begin{subfigure}{0.20\linewidth}
\centering
\includegraphics[width=\textwidth]{figure/rq3/rq3_dt_lime_hr.png}
\vspace{-0.2in}
\caption{SVM}
%\vspace{-0.1in}
\end{subfigure}\hfill

\centering 
\begin{subfigure}{0.20\linewidth}
\centering
\includegraphics[width=\textwidth]{figure/rq3/rq3_dt_lime_rd.png}
\vspace{-0.2in}
\caption{Decision Tree}
%\vspace{-0.1in}
\end{subfigure}\hfill
\begin{subfigure}{0.20\linewidth}
\centering
\includegraphics[width=\textwidth]{figure/rq3/rq3_ens_lime_rd.png}
\vspace{-0.2in}
\caption{Ensemble}
%\vspace{-0.1in}
\end{subfigure}\hfill
\begin{subfigure}{0.20\linewidth}
\centering
\includegraphics[width=\textwidth]{figure/rq3/rq3_gnb_lime_rd.png}
\vspace{-0.2in}
\caption{NaiveBayes}
%\vspace{-0.1in}
\end{subfigure}\hfill
\centering
\begin{subfigure}{0.20\linewidth}
\centering
\includegraphics[width=\textwidth]{figure/rq3/rq3_rf_lime_rd.png}
\vspace{-0.2in}
\caption{RandomForest}
%\vspace{-0.1in}
\end{subfigure}\hfill
\centering
\begin{subfigure}{0.20\linewidth}
\centering
\includegraphics[width=\textwidth]{figure/rq3/rq3_svc_lime_rd.png}
\vspace{-0.2in}
\caption{SVM}
%\vspace{-0.1in}
\end{subfigure}\hfill

\centering 
\begin{subfigure}{0.20\linewidth}
\centering
\includegraphics[width=\textwidth]{figure/rq3/rq3_dt_bd_rd.png}
\vspace{-0.2in}
\caption{Decision Tree}
%\vspace{-0.1in}
\end{subfigure}\hfill
\begin{subfigure}{0.20\linewidth}
\centering
\includegraphics[width=\textwidth]{figure/rq3/rq3_ens_bd_rd.png}
\vspace{-0.2in}
\caption{Ensemble}
%\vspace{-0.1in}
\end{subfigure}\hfill
\begin{subfigure}{0.20\linewidth}
\centering
\includegraphics[width=\textwidth]{figure/rq3/rq3_gnb_bd_rd.png}
\vspace{-0.2in}
\caption{NaiveBayes}
%\vspace{-0.1in}
\end{subfigure}\hfill
\centering
\begin{subfigure}{0.20\linewidth}
\centering
\includegraphics[width=\textwidth]{figure/rq3/rq3_rf_bd_rd.png}
\vspace{-0.2in}
\caption{RandomForest}
%\vspace{-0.1in}
\end{subfigure}\hfill
\centering
\begin{subfigure}{0.20\linewidth}
\centering
\includegraphics[width=\textwidth]{figure/rq3/rq3_svc_bd_rd.png}
\vspace{-0.2in}
\caption{SVM}
%\vspace{-0.1in}
\end{subfigure}\hfill


\vspace{-0.1in}
\caption{ \small
The distributions of {\hitrate} and {\rd} on each project before and after applying data sampling techniques. 
(a) $\sim$ (e) is the result of {\hitrate} of \emph{LIME}.
(f) $\sim$ (j) is the result of {\rd} of \emph{LIME}.
(k) $\sim$ (o) is the result of {\rd} of \emph{BreakDown}.
}
\label{fig:rq3_comb}
\vspace{-0.1in}
\end{figure*}
%\vspace{-0.1in}


==> figure/rq4.tex <==
\begin{figure}
\captionsetup[subfigure]{justification=centering}
    % hit rate part of figure
    \begin{subfigure}[]{\linewidth}
        \begin{tikzpicture}
        \begin{axis}[
        ymax=2,
        ymin=0,
        y=1.5cm,
        xtick={0.0,0.2,0.4,0.6,0.8,1.0},
        xticklabels={0.0,0.2,0.4,0.6,0.8,1.0},
        ytick={1},
        yticklabels={\qquad \, LIME},
        axis y line=left,
        axis x line=bottom,
        xmin=0.0,
        xmax=1.0,
        %ytick={1,2,3},
        %yticklabels={Group A, Group B, Group C},
        ]
        \addplot+[black,thick,
        boxplot prepared={
            draw position=1,
            lower whisker=0.130,
            lower quartile=0.331,
            median=0.549,
            upper quartile=0.624,
            upper whisker=0.810,
        },/pgf/number format/precision=0
        ]
        coordinates {}
        [above]
        node at
        (boxplot box cs: \boxplotvalue{lower whisker},1){}
        node at
        (boxplot box cs: \boxplotvalue{lower quartile},1){}
        node at
        (boxplot box cs: \boxplotvalue{median},1){}
        node at
        (boxplot box cs: \boxplotvalue{upper quartile},1){}
        node at
        (boxplot box cs: \boxplotvalue{upper whisker},1){}
        ;
        
        \end{axis}
        \end{tikzpicture}
        \caption{{\hitrate} of \emph{LIME}}
        \label{fig:rq4_hitrate}
        
    \end{subfigure}

    % rank_diff part of figure
    \begin{subfigure}[]{\linewidth}
        \begin{tikzpicture}
        \begin{axis}[
        ymax=3.5,
        ymin=0,
        y=1.5cm,
        xtick={3,6,...,23},
        xticklabels={3,6,...,23},
        ytick={1,2.5},
        yticklabels={BreakDown, LIME},
        axis y line=left,
        axis x line=bottom,
        xmin=3,
        xmax=23,
        %ytick={1,2,3},
        %yticklabels={Group A, Group B, Group C},
        ]
        \addplot+[black,thick,
        boxplot prepared={
            draw position=2.5,
            lower whisker=3.567,
            lower quartile=5.035,
            median=5.819,
            upper quartile=7.256,
            upper whisker=9.134,
        },/pgf/number format/precision=0
        ]
        coordinates {}
        [above]
        node at
        (boxplot box cs: \boxplotvalue{lower whisker},1){}
        node at
        (boxplot box cs: \boxplotvalue{lower quartile},1){}
        node at
        (boxplot box cs: \boxplotvalue{median},1){}
        node at
        (boxplot box cs: \boxplotvalue{upper quartile},1){}
        node at
        (boxplot box cs: \boxplotvalue{upper whisker},1){}
        ;
         \addplot+[black,thick,
        boxplot prepared={
            draw position=1,
            lower whisker=3.951,
            lower quartile=10.262,
            median=14.330,
            upper quartile=17.333,
            upper whisker=20.840,
        },/pgf/number format/precision=0
        ]
        coordinates {}
        [above]
        node at
        (boxplot box cs: \boxplotvalue{lower whisker},1){}
        node at
        (boxplot box cs: \boxplotvalue{lower quartile},1){}
        node at
        (boxplot box cs: \boxplotvalue{median},1){}
        node at
        (boxplot box cs: \boxplotvalue{upper quartile},1){}
        node at
        (boxplot box cs: \boxplotvalue{upper whisker},1){}
        ;
        
        \end{axis}
        \end{tikzpicture}
        \caption{{\rankdiff} of \emph{LIME} and\emph{BreakDown}} 
        \label{fig:rq4_rankdiff}
    \end{subfigure}
    \caption{Result of RQ4, comparing explanations in cross-project defect prediction scenario}
    \label{fig:rq4}
\end{figure}


==> figure/rq_concept.tex <==
\begin{figure*}
     \centering
         \includegraphics[width=\textwidth]{figure/rq_concept.png}
         \caption{Overall figure of this study}
         \label{fig:rq_concept}
\end{figure*}

==> sec/approach.tex <==
\section{Empirical Study Setup}
\label{sec:approach}


==> sec/contribution.tex <==
\section{*Contribution of Team Members}
\label{sec:contr}
%The contributions of each team member in our project are as following:
\vspace{4pt}
\paragraph{Tasks of Song}
\textbf{Paper Writing}: Abstract, Introduction, Background, Approach, Experiments Setup (4.1),
and Threats. 

\textbf{Project Development}: Craft the idea, Perform defect prediction and static bug finders, 
Implement QATCP algorithm, and Analyze results. 

\vspace{4pt}
\paragraph{Tasks of Yuefei}
\textbf{Paper Writing}: Related Work, Experiments Setup (4.2, 4.3, and 4.4), Results, and Conclusion. 

\textbf{Project Development}: Collect data (i.e., experiment subjects that contain real-world fault, regression fault, and mutation fault), 
Implement benchmark test case prioritization algorithms (i.e., static and dynamic coverage based, similarity based), 
Conduct experiments. 


==> table/different_ks.tex <==
% \begin{table*}[t!]
% \centering
% \caption{Average {\hitrate} and {\rd} of \emph{LIME} with different N features selected when different data sampling techniques are applied.}
% \label{tab:diff_ks}
% \resizebox{0.8\textwidth}{!}{
% \begin{tabular}{c|c|c|c|c|c|c|c|c}
% \hline
% \multirow{2}{*}{\textbf{Project}} & \multicolumn{2}{c|}{\textbf{N = 5}} & \multicolumn{2}{c|}{\textbf{N = 8}} & \multicolumn{2}{c|}{\textbf{N = 10}} & \multicolumn{2}{c}{\textbf{N = 15}} \\ \cline{2-9} 
% & {\hitrate} & {\rd} & {\hitrate} & {\rd} & {\hitrate} & {\rd} & {\hitrate} & {\rd} \\ \hline
% \textbf{Activemq} & 0.463 & 3.168 & 0.529 & 4.787 & 0.569 & 5.711 & 0.681 & 7.039 \\ \hline
% \textbf{Camel} & 0.418 & 3.451 & 0.502 & 5.027 & 0.565 & 5.493 & 0.667 & 7.253 \\ \hline
% \textbf{Derby} & 0.494 & 2.966 & 0.560 & 4.469 & 0.608 & 5.294 & 0.716 & 6.492 \\ \hline
% \textbf{Groovy} & 0.472 & 3.112 & 0.533 & 4.661 & 0.573 & 5.203 & 0.672 & 6.956 \\ \hline
% \textbf{Hbase} & 0.520 & 2.916 & 0.567 & 4.446 & 0.606 & 5.283 & 0.698 & 6.665 \\ \hline
% \textbf{Hive} & 0.486 & 3.094 & 0.556 & 4.578 & 0.583 & 5.500 & 0.679 & 6.925 \\ \hline
% \textbf{Jruby} & 0.417 & 3.430 & 0.509 & 4.915 & 0.549 & 5.862 & 0.660 & 7.247 \\ \hline
% \textbf{Lucene} & 0.494 & 3.070 & 0.576 & 4.094 & 0.595 & 5.352 & 0.676 & 6.836 \\ \hline
% \textbf{Wicket} & 0.456 & 3.161 & 0.552 & 4.616 & 0.600 & 5.465 & 0.719 & 6.551 \\ \hline \hline 
% \textbf{Overall} & 0.469 & 3.150& 0.541 & 4.62& 0.583 &5.463 & 0.685 & 6.885\\ \hline
% \end{tabular}}
% \end{table*}

% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[t!]
\centering
\caption{Average {\hitrate} and {\rd} of \emph{LIME} with different N features selected when different data sampling techniques are applied.}
\label{tab:diff_ks}
%\resizebox{0.7\textwidth}{!}{
\begin{tabular}{c|c|c|c|c|c}
\hline
\multirow{2}{*}{\textbf{Dataset}} & \textbf{N = 5} & \textbf{N = 8} & \textbf{N = 10} & \textbf{N = 15} & \textbf{N = 27/22} \\ \cline{2-6} 
 & \textbf{rank\_diff} & \textbf{rank\_diff} & \textbf{rank\_diff} & \textbf{rank\_diff} & \textbf{rank\_diff} \\ \hline
\textbf{Activemq} & 3.168 & 4.787 & 5.711 & 7.039 & 6.258 \\ \hline
\textbf{Camel} & 3.451 & 5.027 & 5.493 & 7.253 & 6.484 \\ \hline
\textbf{Derby} & 2.966 & 4.469 & 5.294 & 6.492 & 6.013 \\ \hline
\textbf{Groovy} & 3.112 & 4.661 & 5.203 & 6.956 & 6.229 \\ \hline
\textbf{Hbase} & 2.916 & 4.446 & 5.283 & 6.665 & 6.105 \\ \hline
\textbf{Hive} & 3.094 & 4.578 & 5.500 & 6.925 & 6.318 \\ \hline
\textbf{Jruby} & 3.430 & 4.915 & 5.862 & 7.247 & 6.673 \\ \hline
\textbf{Lucene} & 3.070 & 4.094 & 5.352 & 6.836 & 6.476 \\ \hline
\textbf{Wicket} & 3.161 & 4.616 & 5.465 & 6.551 & 5.414 \\ \hline
\end{tabular}%}
\end{table*}

==> table/rq1.tex <==
\begin{table*}[!ht]
\centering
\caption{Result of RQ1, comparison of models with different data sampling techniques applied.} 
%\textbf{``\% of versions''} is the percentage of selected versions from a project.}
\label{tab:rq1}
\begin{subtable}[hbt!]{1\textwidth}
\centering
\resizebox{0.85\textwidth}{!}{
\begin{tabular}{l|l|l|l|l|l|l|l|l|l|l}
\hline
\textbf{LIME (top\_k: 10)} & \multicolumn{2}{l|}{\textbf{Random Under}} & \multicolumn{2}{l|}{\textbf{Repeated Edited NN}} & \multicolumn{2}{l|}{\textbf{Cluster Centroids}} & \multicolumn{2}{l|}{\textbf{SMOTE}} & \multicolumn{2}{l}{\textbf{Random Over}} \\ \hline
Data set & {\hitrate} & {\rd} & {\hitrate} & {\rd} & {\hitrate} & {\rd} & {\hitrate} & {\rd} & {\hitrate} & {\rd} \\ \hline
activemq-5.0.0 & 0.499 & 6.167 & 0.510 & 6.191 & 0.520 & 6.196 & 0.610 & 4.938 & 0.587 & 5.100 \\ \hline
activemq-5.1.0 & 0.530 & 6.269 & 0.623 & 5.278 & 0.573 & 5.634 & 0.641 & 5.238 & 0.642 & 5.108 \\ \hline
activemq-5.2.0 & 0.480 & 6.548 & 0.545 & 5.970 & 0.518 & 6.091 & 0.534 & 6.044 & 0.422 & 6.847 \\ \hline
activemq-5.3.0 & 0.540 & 6.280 & 0.555 & 6.096 & 0.560 & 5.807 & 0.654 & 4.918 & 0.672 & 4.921 \\ \hline
activemq-5.8.0 & 0.597 & 5.574 & 0.618 & 5.688 & 0.528 & 5.880 & 0.590 & 5.117 & 0.661 & 4.294 \\ \hline
camel-1.4.0 & 0.610 & 5.086 & 0.579 & 5.279 & 0.574 & 5.285 & 0.715 & 3.909 & 0.696 & 4.311 \\ \hline
camel-2.9.0 & 0.620 & 5.222 & 0.603 & 5.643 & 0.481 & 6.303 & 0.779 & 3.971 & 0.728 & 4.274 \\ \hline
camel-2.10.0 & 0.582 & 5.660 & 0.734 & 4.097 & 0.498 & 6.583 & 0.775 & 3.750 & 0.764 & 3.577 \\ \hline
camel-2.11.0 & 0.549 & 5.917 & 0.529 & 6.176 & 0.401 & 7.336 & 0.766 & 4.485 & 0.765 & 4.491 \\ \hline
derby-10.2.1.6 & 0.372 & 6.759 & 0.332 & 7.233 & 0.378 & 6.601 & 0.367 & 6.752 & 0.383 & 6.558 \\ \hline
derby-10.3.1.4 & 0.365 & 6.854 & 0.327 & 7.384 & 0.359 & 6.824 & 0.360 & 6.887 & 0.356 & 6.909 \\ \hline
derby-10.5.1.1 & 0.350 & 7.039 & 0.332 & 7.098 & 0.359 & 6.824 & 0.330 & 7.249 & 0.322 & 7.269 \\ \hline
groovy-1\_5\_7 & 0.473 & 6.644 & 0.498 & 6.505 & 0.307 & 7.281 & 0.657 & 5.402 & 0.640 & 5.641 \\ \hline
groovy-1\_6\_BETA\_1 & 0.523 & 6.146 & 0.545 & 5.673 & 0.605 & 5.418 & 0.601 & 5.300 & 0.657 & 4.744 \\ \hline
groovy-1\_6\_BETA\_2 & 0.635 & 4.783 & 0.564 & 5.331 & 0.469 & 6.263 & 0.684 & 4.504 & 0.689 & 4.272 \\ \hline
hbase-0.94.0 & 0.553 & 5.739 & 0.510 & 5.953 & 0.569 & 5.491 & 0.589 & 5.281 & 0.603 & 4.989 \\ \hline
hbase-0.95.0 & 0.679 & 4.258 & 0.665 & 4.745 & 0.670 & 4.632 & 0.700 & 4.015 & 0.723 & 3.888 \\ \hline
hbase-0.95.2 & 0.603 & 5.065 & 0.595 & 4.974 & 0.625 & 4.718 & 0.614 & 4.706 & 0.619 & 4.816 \\ \hline
hive-0.9.0 & 0.736 & 4.492 & 0.721 & 5.098 & 0.765 & 4.070 & 0.802 & 3.361 & 0.748 & 4.221 \\ \hline
hive-0.10.0 & 0.592 & 5.408 & 0.594 & 5.254 & 0.557 & 5.401 & 0.609 & 5.022 & 0.576 & 5.208 \\ \hline
hive-0.12.0 & 0.474 & 6.632 & 0.632 & 5.244 & 0.693 & 4.614 & 0.249 & 8.286 & 0.418 & 6.399 \\ \hline
jruby-1.1 & 0.613 & 5.074 & 0.625 & 4.674 & 0.615 & 4.782 & 0.667 & 4.539 & 0.675 & 4.453 \\ \hline
jruby-1.4.0 & 0.644 & 4.723 & 0.709 & 4.021 & 0.661 & 4.683 & 0.645 & 4.712 & 0.674 & 4.552 \\ \hline
jruby-1.5.0 & 0.322 & 7.265 & 0.347 & 7.171 & 0.338 & 7.065 & 0.369 & 6.845 & 0.295 & 7.681 \\ \hline
jruby-1.7.0.preview1 & 0.624 & 4.960 & 0.767 & 3.538 & 0.535 & 5.567 & 0.613 & 4.905 & 0.594 & 5.154 \\ \hline
lucene-2.3.0 & 0.431 & 6.489 & 0.407 & 6.854 & 0.418 & 6.407 & 0.388 & 6.961 & 0.422 & 6.519 \\ \hline
lucene-2.9.0 & 0.406 & 6.496 & 0.445 & 6.114 & 0.390 & 6.755 & 0.424 & 6.453 & 0.403 & 6.625 \\ \hline
lucene-3.0.0 & 0.552 & 5.978 & 0.549 & 5.435 & 0.521 & 5.629 & 0.540 & 5.755 & 0.491 & 6.208 \\ \hline
lucene-3.1 & 0.421 & 6.370 & 0.452 & 6.279 & 0.380 & 6.744 & 0.377 & 6.786 & 0.356 & 6.971 \\ \hline
wicket-1.3.0-beta2 & 0.436 & 6.552 & 0.564 & 5.577 & 0.636 & 4.717 & 0.519 & 6.218 & 0.691 & 4.286 \\ \hline
wicket-1.3.0-incubating-beta-1 & 0.575 & 6.020 & 0.567 & 5.900 & 0.690 & 4.729 & 0.614 & 5.133 & 0.668 & 4.761 \\ \hline
wicket-1.5.3 & 0.436 & 6.552 & 0.564 & 5.577 & 0.518 & 5.658 & 0.519 & 6.218 & 0.594 & 5.126 \\ \hline \hline
average & 0.526	& 5.907	& 0.550	& 5.689	& 0.522	& 5.812	& 0.572	& 5.427	& 0.579	& 5.318 \\ \hline
\end{tabular}}
\caption{Result of Lime}
\label{tab:rq1_lime}

\centering
\resizebox{0.7\textwidth}{!}{
\begin{tabular}{l|l|l|l|l|l}
\hline
\textbf{BreakDown} & \textbf{Random Under} & \textbf{RepeatedEditedNN} & \textbf{Cluster Centroid} & \textbf{SMOTE} & \textbf{Random Over} \\ \hline
Data set & {\rd} & {\rd} & {\rd} & {\rd} & {\rd} \\ \hline
activemq-5.0.0 & 12.846 & 12.011 & 13.213 & 9.273 & 10.141 \\ \hline
activemq-5.1.0 & 14.035 & 10.158 & 13.047 & 9.631 & 9.444 \\ \hline
activemq-5.2.0 & 13.725 & 9.190 & 12.130 & 9.794 & 12.177 \\ \hline
activemq-5.3.0 & 13.776 & 12.315 & 11.387 & 6.864 & 6.226 \\ \hline
activemq-5.8.0 & 15.516 & 12.298 & 17.510 & 15.458 & 12.872 \\ \hline
camel-1.4.0 & 10.263 & 14.841 & 11.010 & 6.531 & 6.068 \\ \hline
camel-2.9.0 & 15.799 & 14.932 & 17.798 & 10.163 & 12.053 \\ \hline
camel-2.10.0 & 14.953 & 7.995 & 17.477 & 8.740 & 7.852 \\ \hline
camel-2.11.0 & 14.435 & 11.794 & 17.850 & 8.318 & 8.014 \\ \hline
derby-10.2.1.6 & 11.057 & 16.629 & 9.912 & 10.573 & 10.538 \\ \hline
derby-10.3.1.4 & 13.407 & 14.787 & 11.980 & 13.103 & 13.179 \\ \hline
derby-10.5.1.1 & 30.768 & 23.622 & 11.980 & 30.260 & 29.913 \\ \hline
groovy-1\_5\_7 & 17.824 & 14.109 & 25.660 & 12.610 & 11.769 \\ \hline
groovy-1\_6\_BETA\_1 & 14.993 & 13.419 & 17.466 & 11.396 & 11.400 \\ \hline
groovy-1\_6\_BETA\_2 & 13.113 & 15.767 & 13.828 & 8.391 & 9.805 \\ \hline
hbase-0.94.0 & 11.230 & 15.892 & 10.205 & 10.389 & 8.654 \\ \hline
hbase-0.95.0 & 9.526 & 13.912 & 11.389 & 7.619 & 8.248 \\ \hline
hbase-0.95.2 & 9.499 & 11.833 & 7.605 & 8.008 & 7.993 \\ \hline
hive-0.9.0 & 9.525 & 14.868 & 9.171 & 5.506 & 5.529 \\ \hline
hive-0.10.0 & 12.679 & 16.721 & 17.274 & 21.125 & 20.744 \\ \hline
hive-0.12.0 & 16.634 & 15.524 & 15.015 & 22.747 & 22.847 \\ \hline
jruby-1.1 & 13.616 & 13.867 & 12.661 & 6.838 & 8.024 \\ \hline
jruby-1.4.0 & 11.471 & 15.420 & 12.257 & 8.342 & 7.914 \\ \hline
jruby-1.5.0 & 19.345 & 21.558 & 22.428 & 28.776 & 28.820 \\ \hline
jruby-1.7.0.preview1 & 13.597 & 6.123 & 19.962 & 10.212 & 13.167 \\ \hline
lucene-2.3.0 & 23.679 & 17.670 & 11.901 & 22.809 & 24.242 \\ \hline
lucene-2.9.0 & 19.768 & 16.680 & 17.425 & 25.349 & 25.444 \\ \hline
lucene-3.0.0 & 15.252 & 8.356 & 18.586 & 17.474 & 15.487 \\ \hline
lucene-3.1 & 25.741 & 15.609 & 14.209 & 27.745 & 27.684 \\ \hline
wicket-1.3.0-beta2 & 14.989 & 8.164 & 14.627 & 12.434 & 10.431 \\ \hline
wicket-1.3.0-incubating-beta-1 & 12.371 & 9.098 & 13.031 & 14.005 & 7.723 \\ \hline
wicket-1.5.3 & 14.614 & 8.164 & 14.627 & 12.194 & 9.317 \\ \hline \hline
average & 15.001 & 13.541 & 14.520 & 13.521 & 13.241 \\ \hline
\end{tabular}}
\caption{Result of BreakDown}
\label{tab:rq1_bd}

\end{subtable}
\end{table*}



==> table/rq2.tex <==
\begin{table*}[!ht]
\centering
\caption{Result of RQ2, comparison of different machine learning algorithms } 
%\textbf{``\% of versions''} is the percentage of selected versions from a project.}
\label{tab:rq2}
\begin{subtable}[hbt!]{1\textwidth}
\centering
\resizebox{0.8\textwidth}{!}{
\begin{tabular}{l|l|l|l|l|l|l|l|l|l|l}
\hline
LIME  & \multicolumn{2}{l|}{SVM} & \multicolumn{2}{l|}{NB (Gaussian)} & \multicolumn{2}{l|}{RF} & \multicolumn{2}{l|}{Ensemble(Adaboost)} & \multicolumn{2}{l}{DT} \\ \hline
Data sets & {\hitrate}  & {\rd} & {\hitrate} & {\rd} & {\hitrate}  & {\rd} & {\hitrate}  & {\rd} & {\hitrate}  & {\rd} \\ \hline
activemq-5.0.0 & 0.360 & 7.380 & 0.308 & 8.077  & 0.292  & 7.930  & 0.258  & 8.213  & 0.249  & 8.441  \\ \hline
activemq-5.1.0 & N/A & N/A & 0.277 & 7.957  & 0.331  & 7.759  & 0.225  & 8.101  & 0.242  & 8.360  \\ \hline
activemq-5.2.0 & N/A & N/A & 0.461 & 6.520  & 0.104  & 9.284  & 0.202  & 8.476  & 0.119  & 9.242  \\ \hline
activemq-5.3.0 & 0.267 & 8.233 & 0.218 & 8.711  & 0.257  & 8.093  & 0.157  & 9.012  & 0.190  & 8.794  \\ \hline
activemq-5.8.0 & N/A & N/A & 0.297 & 7.588  & 0.219  & 8.471  & 0.247  & 8.236  & 0.172  & 8.725  \\ \hline
camel-1.4.0  & 0.467 & 7.117 & 0.389 & 7.037  & 0.239  & 8.330  & 0.201  & 8.682  & 0.258  & 8.220  \\ \hline
camel-2.9.0  & N/A & N/A & 0.597 & 5.361  & 0.475  & 6.688  & 0.270  & 8.100  & 0.250  & 8.404  \\ \hline
camel-2.10.0 & N/A & N/A & 0.306 & 8.035  & 0.325  & 7.688  & 0.156  & 8.756  & 0.250  & 8.248  \\ \hline
camel-2.11.0 & N/A & N/A & 0.444 & 6.982  & 0.200  & 8.900  & 0.200  & 9.100  & 0.325  & 7.738  \\ \hline
derby-10.2.1.6 & 0.357 & 6.821 & 0.384 & 6.610  & 0.185  & 8.692  & 0.215  & 8.496  & 0.204  & 8.551  \\ \hline
derby-10.3.1.4 & 0.329 & 7.057 & 0.377 & 6.712  & 0.148  & 9.006  & 0.245  & 8.368  & 0.209  & 8.551  \\ \hline
derby-10.5.1.1 & 0.320 & 7.400 & 0.420 & 6.653  & 0.134  & 9.174  & 0.171  & 8.855  & 0.171  & 8.971  \\ \hline
groovy-1\_5\_7 & N/A & N/A & 0.347 & 7.520  & 0.270  & 8.300  & 0.287  & 7.963  & 0.081  & 9.506  \\ \hline
groovy-1\_6\_BETA\_1 & N/A & N/A & 0.408 & 6.806  & 0.331  & 7.770  & 0.222  & 8.296  & 0.233  & 8.317  \\ \hline
groovy-1\_6\_BETA\_2 & 0.200 & 8.100 & 0.399 & 6.667  & 0.170  & 9.095  & 0.170  & 8.880  & 0.185  & 8.848  \\ \hline
hbase-0.94.0 & 0.300 & 8.300 & 0.591 & 5.628  & 0.223  & 8.442  & 0.129  & 9.141  & 0.178  & 8.749  \\ \hline
hbase-0.95.0 & 0.200 & 8.300 & 0.233 & 7.933  & 0.108  & 9.183  & 0.237  & 8.328  & 0.140  & 9.116  \\ \hline
hbase-0.95.2 & 0.200 & 8.500 & 0.253 & 7.767  & 0.187  & 8.558  & 0.321  & 7.784  & 0.156  & 9.045  \\ \hline
hive-0.9.0 & 0.204 & 8.796 & 0.753 & 4.734  & 0.488  & 6.384  & 0.266  & 8.218  & 0.232  & 8.447  \\ \hline
hive-0.10.0  & 0.200 & 8.375 & 0.520 & 5.580  & 0.350  & 7.917  & 0.233  & 8.743  & 0.347  & 7.839  \\ \hline
hive-0.12.0  & N/A & N/A & 0.650 & 4.912  & 0.300  & 7.700  & 0.400  & 7.900  & 0.300  & 8.050  \\ \hline
jruby-1.1 & 0.200 & 8.100 & 0.260 & 7.600  & 0.223  & 8.716  & 0.285  & 8.095  & 0.145  & 9.058  \\ \hline
jruby-1.4.0  & 0.233 & 8.200 & 0.275 & 7.429  & 0.289  & 8.004  & 0.192  & 8.434  & 0.194  & 8.713  \\ \hline
jruby-1.5.0  & 0.325 & 7.600 & 0.375 & 6.738  & 0.140  & 9.290  & 0.225  & 8.790  & 0.194  & 8.678  \\ \hline
jruby-1.7.0.preview1 & N/A & N/A & 0.464 & 6.171  & 0.290  & 7.920  & 0.378  & 7.433  & 0.273  & 8.225  \\ \hline
lucene-2.3.0 & N/A & N/A & 0.460 & 5.973  & 0.173  & 8.863  & 0.223  & 8.586  & 0.233  & 8.445  \\ \hline
lucene-2.9.0 & 0.400 & 7.100 & 0.275 & 7.500  & 0.208  & 8.658  & 0.231  & 8.450  & 0.210  & 8.670  \\ \hline
lucene-3.0.0 & N/A & N/A & 0.267 & 7.633  & 0.233  & 8.533  & 0.267  & 8.411  & 0.267  & 8.100  \\ \hline
lucene-3.1 & N/A & N/A & 0.467 & 6.167  & 0.100  & 9.200  & 0.233  & 8.400  & 0.204  & 8.598  \\ \hline
wicket-1.3.0-beta2 & N/A & N/A & 0.419 & 6.527  & 0.333  & 7.849  & 0.261  & 8.310  & 0.245  & 8.340  \\ \hline
wicket-1.3.0-incubating-beta-1 & N/A & N/A & 0.418 & 6.590  & 0.175  & 8.881  & 0.252  & 8.256  & 0.168  & 9.024  \\ \hline
wicket-1.5.3 & N/A & N/A & 0.518 & 6.021  & 0.280  & 7.880  & 0.231  & 8.474  & 0.197  & 8.739  \\ \hline \hline
average & 0.285 & 7.836 & 0.401 & 6.817 & 0.243 & 8.349 & 0.237 & 8.415 & 0.213 & 8.586 \\ \hline
\end{tabular}}
\caption{Result of Lime}
\label{tab:rq2_lime}

\centering
\resizebox{0.55\textwidth}{!}{
\begin{tabular}{l|l|l|l|l|l}
\hline
BreakDown & SVM & NB & RF & Ensemble & DT \\ \hline
Data set  & {\rd} & {\rd} & {\rd} & {\rd} & {\rd} \\ \hline
activemq-5.0.0 & 15.506 & 19.632 & 20.572 & 18.892 & 20.415 \\ \hline
activemq-5.1.0 & N/A & 19.516 & 19.184 & 21.686 & 21.376 \\ \hline
activemq-5.2.0 & N/A & 20.293 & 18.999 & 17.582 & 19.286 \\ \hline
activemq-5.3.0 & 15.015 & 19.128 & 19.212 & 20.049 & 19.606 \\ \hline
activemq-5.8.0 & N/A & 22.520 & 22.677 & 20.527 & 21.596 \\ \hline
camel-1.4.0  & 17.236 & 19.176 & 18.877 & 19.857 & 20.251 \\ \hline
camel-2.9.0  & N/A & 18.846 & 20.137 & 18.283 & 21.006 \\ \hline
camel-2.10.0 & N/A & 16.821 & 19.158 & 20.282 & 20.056 \\ \hline
camel-2.11.0 & N/A & 16.633 & 17.754 & 19.600 & 17.635 \\ \hline
derby-10.2.1.6 & 12.454 & 11.409 & 17.675 & 20.671 & 19.512 \\ \hline
derby-10.3.1.4 & 16.114 & 14.860 & 18.814 & 21.447 & 21.141 \\ \hline
derby-10.5.1.1 & 30.468 & 31.042 & 30.030 & 22.971 & 26.149 \\ \hline
groovy-1\_5\_7 & N/A & 20.697 & 21.418 & 20.486 & 22.056 \\ \hline
groovy-1\_6\_BETA\_1 & N/A & 23.099 & 21.947 & 19.394 & 21.050 \\ \hline
groovy-1\_6\_BETA\_2 & 11.692 & 22.562 & 20.163 & 19.872 & 20.403 \\ \hline
hbase-0.94.0 & 15.323 & 21.630 & 22.351 & 19.369 & 20.312 \\ \hline
hbase-0.95.0 & 18.538 & 20.487 & 21.834 & 19.576 & 21.818 \\ \hline
hbase-0.95.2 & 18.092 & 21.187 & 21.377 & 19.421 & 20.378 \\ \hline
hive-0.9.0 & 18.694 & 19.031 & 19.982 & 21.200 & 20.033 \\ \hline
hive-0.10.0  & 15.808 & 22.138 & 20.558 & 19.649 & 21.521 \\ \hline
hive-0.12.0  & N/A & 24.107 & 23.785 & 22.954 & 19.477 \\ \hline
jruby-1.1 & 22.892 & 20.945 & 20.774 & 19.320 & 21.124 \\ \hline
jruby-1.4.0  & 21.041 & 21.067 & 21.908 & 19.448 & 22.109 \\ \hline
jruby-1.5.0  & 29.046 & 27.131 & 29.692 & 22.329 & 23.019 \\ \hline
jruby-1.7.0.preview1 & N/A & 20.765 & 23.582 & 19.275 & 21.260 \\ \hline
lucene-2.3.0 & N/A & 26.658 & 23.277 & 20.349 & 22.034 \\ \hline
lucene-2.9.0 & 25.908 & 26.292 & 27.333 & 22.568 & 24.386 \\ \hline
lucene-3.0.0 & N/A & 21.938 & 20.400 & 20.701 & 21.067 \\ \hline
lucene-3.1 & N/A & 27.908 & 22.246 & 19.713 & 20.822 \\ \hline
wicket-1.3.0-beta2 & N/A & 20.245 & 20.607 & 20.133 & 20.963 \\ \hline
wicket-1.3.0-incubating-beta-1 & N/A & 18.926 & 19.612 & 18.186 & 20.249 \\ \hline
wicket-1.5.3 & N/A & 18.280 & 17.600 & 17.886 & 18.911 \\ \hline \hline
average & 18.989 & 21.093 & 21.360 & 20.115 & 20.969 \\ \hline
\end{tabular}}
\caption{Result of BreakDown}
\label{tab:rq2_bd}

\end{subtable}
\end{table*}


